On Latency Predictors for Neural Architecture Search

Efficient deployment of neural networks (NN) requires the co-optimization of accuracy and latency. For example, hardware-aware neural architecture search has been used to automatically find NN architectures that satisfy a latency constraint on a specific hardware device. Central to these search algorithms is a prediction model that is designed to provide a hardware latency estimate for a candidate NN architecture. Recent research has shown that the sample efficiency of these predictive models can be greatly improved through pre-training on some \textit{training} devices with many samples, and then transferring the predictor on the \textit{test} (target) device. Transfer learning and meta-learning methods have been used for this, but often exhibit significant performance variability. Additionally, the evaluation of existing latency predictors has been largely done on hand-crafted training/test device sets, making it difficult to ascertain design features that compose a robust and general latency predictor. To address these issues, we introduce a comprehensive suite of latency prediction tasks obtained in a principled way through automated partitioning of hardware device sets. We then design a general latency predictor to comprehensively study (1) the predictor architecture, (2) NN sample selection methods, (3) hardware device representations, and (4) NN operation encoding schemes. Building on conclusions from our study, we present an end-to-end latency predictor training strategy that outperforms existing methods on 11 out of 12 difficult latency prediction tasks, improving latency prediction by 22.5\% on average, and up to to 87.6\% on the hardest tasks. Focusing on latency prediction, our HW-Aware NAS reports a $5.8\times$ speedup in wall-clock time. Our code is available on \href{https://github.com/abdelfattah-lab/nasflat_latency}{https://github.com/abdelfattah-lab/nasflat\_latency}.

==> appxfgs/fb_allcorr.tex <==


\begin{table*}[h!]
    \centering
    \resizebox{\linewidth}{!}{%

\begin{tabular}{llllllllllllllllllllllllllll}
\toprule
{} & 1080ti\_1 & 1080ti\_32 & 1080ti\_64 & 2080ti\_1 & 2080ti\_32 & 2080ti\_64 & essential\_ph\_1 & eyeriss &   fpga & gold\_6226 & gold\_6240 & pixel2 & pixel3 & raspi4 & samsung\_a50 & samsung\_s7 & silver\_4114 & silver\_4210r & titan\_rtx\_1 & titan\_rtx\_32 & titan\_rtx\_64 & titanx\_1 & titanx\_32 & titanx\_64 & titanxp\_1 & titanxp\_32 & titanxp\_64 \\
\midrule
1080ti\_1        &     1.000 &      0.764 &      0.439 &     0.944 &      0.799 &      0.496 &            0.258 &   0.247 &  0.226 &      0.207 &      0.536 &  0.300 &  0.249 &  0.256 &        0.320 &       0.307 &        0.576 &         0.653 &         0.948 &          0.846 &          0.590 &     0.946 &      0.687 &      0.423 &      0.946 &       0.756 &       0.490 \\
1080ti\_32       &     0.764 &      1.000 &      0.817 &     0.811 &      0.966 &      0.853 &            0.338 &   0.527 &  0.419 &      0.241 &      0.459 &  0.409 &  0.555 &  0.524 &        0.478 &       0.372 &        0.488 &         0.559 &         0.815 &          0.955 &          0.911 &     0.808 &      0.953 &      0.801 &      0.805 &       0.971 &       0.856 \\
1080ti\_64       &     0.439 &      0.817 &      1.000 &     0.469 &      0.806 &      0.985 &            0.414 &   0.757 &  0.605 &      0.323 &      0.350 &  0.496 &  0.795 &  0.719 &        0.595 &       0.421 &        0.355 &         0.401 &         0.475 &          0.741 &          0.965 &     0.472 &      0.910 &      0.985 &      0.468 &       0.858 &       0.991 \\
2080ti\_1        &     0.944 &      0.811 &      0.469 &     1.000 &      0.848 &      0.530 &            0.240 &   0.238 &  0.206 &      0.178 &      0.524 &  0.287 &  0.243 &  0.241 &        0.310 &       0.293 &        0.567 &         0.650 &         0.991 &          0.896 &          0.629 &     0.985 &      0.729 &      0.453 &      0.985 &       0.801 &       0.524 \\
2080ti\_32       &     0.799 &      0.966 &      0.806 &     0.848 &      1.000 &      0.851 &            0.312 &   0.489 &  0.385 &      0.214 &      0.449 &  0.388 &  0.519 &  0.492 &        0.455 &       0.349 &        0.483 &         0.559 &         0.850 &          0.984 &          0.914 &     0.841 &      0.958 &      0.789 &      0.838 &       0.981 &       0.847 \\
2080ti\_64       &     0.496 &      0.853 &      0.985 &     0.530 &      0.851 &      1.000 &            0.395 &   0.723 &  0.582 &      0.297 &      0.350 &  0.485 &  0.754 &  0.688 &        0.581 &       0.406 &        0.360 &         0.412 &         0.534 &          0.787 &          0.986 &     0.529 &      0.936 &      0.974 &      0.525 &       0.891 &       0.992 \\
essential\_ph\_1 &     0.258 &      0.338 &      0.414 &     0.240 &      0.312 &      0.395 &            1.000 &   0.678 &  0.700 &      0.670 &      0.663 &  0.635 &  0.646 &  0.660 &        0.646 &       0.650 &        0.613 &         0.608 &         0.268 &          0.313 &          0.388 &     0.300 &      0.379 &      0.427 &      0.286 &       0.362 &       0.406 \\
eyeriss          &     0.247 &      0.527 &      0.757 &     0.238 &      0.489 &      0.723 &            0.678 &   1.000 &  0.941 &      0.796 &      0.666 &  0.767 &  0.976 &  0.952 &        0.864 &       0.690 &        0.624 &         0.633 &         0.249 &          0.442 &          0.674 &     0.279 &      0.617 &      0.773 &      0.269 &       0.559 &       0.731 \\
fpga             &     0.226 &      0.419 &      0.605 &     0.206 &      0.385 &      0.582 &            0.700 &   0.941 &  1.000 &      0.868 &      0.723 &  0.781 &  0.906 &  0.913 &        0.865 &       0.713 &        0.674 &         0.679 &         0.217 &          0.350 &          0.534 &     0.255 &      0.489 &      0.623 &      0.245 &       0.442 &       0.580 \\
gold\_6226       &     0.207 &      0.241 &      0.323 &     0.178 &      0.214 &      0.297 &            0.670 &   0.796 &  0.868 &      1.000 &      0.820 &  0.747 &  0.741 &  0.796 &        0.805 &       0.697 &        0.758 &         0.752 &         0.184 &          0.209 &          0.274 &     0.232 &      0.270 &      0.344 &      0.222 &       0.250 &       0.303 \\
gold\_6240       &     0.536 &      0.459 &      0.350 &     0.524 &      0.449 &      0.350 &            0.663 &   0.666 &  0.723 &      0.820 &      1.000 &  0.678 &  0.619 &  0.679 &        0.732 &       0.688 &        0.916 &         0.940 &         0.536 &          0.481 &          0.383 &     0.578 &      0.436 &      0.362 &      0.568 &       0.459 &       0.360 \\
pixel2           &     0.300 &      0.409 &      0.496 &     0.287 &      0.388 &      0.485 &            0.635 &   0.767 &  0.781 &      0.747 &      0.678 &  1.000 &  0.729 &  0.747 &        0.735 &       0.629 &        0.643 &         0.653 &         0.296 &          0.369 &          0.466 &     0.328 &      0.449 &      0.512 &      0.318 &       0.425 &       0.486 \\
pixel3           &     0.249 &      0.555 &      0.795 &     0.243 &      0.519 &      0.754 &            0.646 &   0.976 &  0.906 &      0.741 &      0.619 &  0.729 &  1.000 &  0.957 &        0.828 &       0.655 &        0.584 &         0.598 &         0.253 &          0.471 &          0.708 &     0.278 &      0.650 &      0.810 &      0.270 &       0.590 &       0.770 \\
raspi4           &     0.256 &      0.524 &      0.719 &     0.241 &      0.492 &      0.688 &            0.660 &   0.952 &  0.913 &      0.796 &      0.679 &  0.747 &  0.957 &  1.000 &        0.841 &       0.678 &        0.641 &         0.649 &         0.251 &          0.450 &          0.648 &     0.286 &      0.607 &      0.733 &      0.276 &       0.555 &       0.698 \\
samsung\_a50     &     0.320 &      0.478 &      0.595 &     0.310 &      0.455 &      0.581 &            0.646 &   0.864 &  0.865 &      0.805 &      0.732 &  0.735 &  0.828 &  0.841 &        1.000 &       0.684 &        0.686 &         0.698 &         0.317 &          0.429 &          0.556 &     0.352 &      0.531 &      0.609 &      0.341 &       0.498 &       0.582 \\
samsung\_s7      &     0.307 &      0.372 &      0.421 &     0.293 &      0.349 &      0.406 &            0.650 &   0.690 &  0.713 &      0.697 &      0.688 &  0.629 &  0.655 &  0.678 &        0.684 &       1.000 &        0.649 &         0.653 &         0.312 &          0.352 &          0.404 &     0.347 &      0.402 &      0.435 &      0.337 &       0.388 &       0.416 \\
silver\_4114     &     0.576 &      0.488 &      0.355 &     0.567 &      0.483 &      0.360 &            0.613 &   0.624 &  0.674 &      0.758 &      0.916 &  0.643 &  0.584 &  0.641 &        0.686 &       0.649 &        1.000 &         0.941 &         0.580 &          0.519 &          0.402 &     0.619 &      0.459 &      0.367 &      0.610 &       0.489 &       0.369 \\
silver\_4210r    &     0.653 &      0.559 &      0.401 &     0.650 &      0.559 &      0.412 &            0.608 &   0.633 &  0.679 &      0.752 &      0.940 &  0.653 &  0.598 &  0.649 &        0.698 &       0.653 &        0.941 &         1.000 &         0.659 &          0.596 &          0.459 &     0.694 &      0.522 &      0.410 &      0.686 &       0.557 &       0.419 \\
titan\_rtx\_1    &     0.948 &      0.815 &      0.475 &     0.991 &      0.850 &      0.534 &            0.268 &   0.249 &  0.217 &      0.184 &      0.536 &  0.296 &  0.253 &  0.251 &        0.317 &       0.312 &        0.580 &         0.659 &         1.000 &          0.899 &          0.635 &     0.991 &      0.735 &      0.460 &      0.991 &       0.807 &       0.531 \\
titan\_rtx\_32   &     0.846 &      0.955 &      0.741 &     0.896 &      0.984 &      0.787 &            0.313 &   0.442 &  0.350 &      0.209 &      0.481 &  0.369 &  0.471 &  0.450 &        0.429 &       0.352 &        0.519 &         0.596 &         0.899 &          1.000 &          0.864 &     0.892 &      0.927 &      0.724 &      0.889 &       0.966 &       0.788 \\
titan\_rtx\_64   &     0.590 &      0.911 &      0.965 &     0.629 &      0.914 &      0.986 &            0.388 &   0.674 &  0.534 &      0.274 &      0.383 &  0.466 &  0.708 &  0.648 &        0.556 &       0.404 &        0.402 &         0.459 &         0.635 &          0.864 &          1.000 &     0.629 &      0.973 &      0.951 &      0.624 &       0.945 &       0.983 \\
titanx\_1        &     0.946 &      0.808 &      0.472 &     0.985 &      0.841 &      0.529 &            0.300 &   0.279 &  0.255 &      0.232 &      0.578 &  0.328 &  0.278 &  0.286 &        0.352 &       0.347 &        0.619 &         0.694 &         0.991 &          0.892 &          0.629 &     1.000 &      0.729 &      0.458 &      0.991 &       0.801 &       0.526 \\
titanx\_32       &     0.687 &      0.953 &      0.910 &     0.729 &      0.958 &      0.936 &            0.379 &   0.617 &  0.489 &      0.270 &      0.436 &  0.449 &  0.650 &  0.607 &        0.531 &       0.402 &        0.459 &         0.522 &         0.735 &          0.927 &          0.973 &     0.729 &      1.000 &      0.895 &      0.725 &       0.981 &       0.939 \\
titanx\_64       &     0.423 &      0.801 &      0.985 &     0.453 &      0.789 &      0.974 &            0.427 &   0.773 &  0.623 &      0.344 &      0.362 &  0.512 &  0.810 &  0.733 &        0.609 &       0.435 &        0.367 &         0.410 &         0.460 &          0.724 &          0.951 &     0.458 &      0.895 &      1.000 &      0.453 &       0.841 &       0.981 \\
titanxp\_1       &     0.946 &      0.805 &      0.468 &     0.985 &      0.838 &      0.525 &            0.286 &   0.269 &  0.245 &      0.222 &      0.568 &  0.318 &  0.270 &  0.276 &        0.341 &       0.337 &        0.610 &         0.686 &         0.991 &          0.889 &          0.624 &     0.991 &      0.725 &      0.453 &      1.000 &       0.797 &       0.521 \\
titanxp\_32      &     0.756 &      0.971 &      0.858 &     0.801 &      0.981 &      0.891 &            0.362 &   0.559 &  0.442 &      0.250 &      0.459 &  0.425 &  0.590 &  0.555 &        0.498 &       0.388 &        0.489 &         0.557 &         0.807 &          0.966 &          0.945 &     0.801 &      0.981 &      0.841 &      0.797 &       1.000 &       0.895 \\
titanxp\_64      &     0.490 &      0.856 &      0.991 &     0.524 &      0.847 &      0.992 &            0.406 &   0.731 &  0.580 &      0.303 &      0.360 &  0.486 &  0.770 &  0.698 &        0.582 &       0.416 &        0.369 &         0.419 &         0.531 &          0.788 &          0.983 &     0.526 &      0.939 &      0.981 &      0.521 &       0.895 &       1.000 \\
\bottomrule
\end{tabular}

    
}
\caption{Device correlations}
\label{tab:fballdevcor}
\end{table*}

==> appxfgs/nb2_allcorr.tex <==


\begin{table*}[h!]
    \centering
    \resizebox{\linewidth}{!}{%


\begin{tabular}{lllllllllllllllllllllllllllllllllllllllll}
\toprule
{} & 1080ti\_1 & 1080ti\_256 & 1080ti\_32 & 2080ti\_1 & 2080ti\_256 & 2080ti\_32 & d\_cpu\_core\_i7\_7820x\_fp32 & d\_gpu\_gtx\_1080ti\_fp32 & e\_gpu\_jetson\_nano\_fp16 & e\_gpu\_jetson\_nano\_fp32 & e\_tpu\_edge\_tpu\_int8 & essential\_ph\_1 & eyeriss &   fpga & gold\_6226 & gold\_6240 & m\_cpu\_sd\_450\_cortex\_a53\_int8 & m\_cpu\_sd\_675\_kryo\_460\_int8 & m\_cpu\_sd\_855\_kryo\_485\_int8 & m\_dsp\_sd\_675\_hexagon\_685\_int8 & m\_dsp\_sd\_855\_hexagon\_690\_int8 & m\_gpu\_sd\_450\_adreno\_506\_int8 & m\_gpu\_sd\_675\_adreno\_612\_int8 & m\_gpu\_sd\_855\_adreno\_640\_int8 & pixel2 & pixel3 & raspi4 & samsung\_a50 & samsung\_s7 & silver\_4114 & silver\_4210r & titan\_rtx\_1 & titan\_rtx\_256 & titan\_rtx\_32 & titanx\_1 & titanx\_256 & titanx\_32 & titanxp\_1 & titanxp\_256 & titanxp\_32 \\
\midrule
1080ti\_1                           &     1.000 &       0.741 &      0.971 &     0.965 &       0.780 &      0.981 &                         0.360 &                     0.362 &                      0.514 &                      0.739 &                   0.167 &            0.842 &   0.415 &  0.828 &      0.958 &      0.831 &                              0.670 &                            0.636 &                            0.645 &                               0.593 &                               0.587 &                              0.610 &                              0.594 &                              0.551 &  0.807 &  0.591 &  0.654 &        0.804 &       0.887 &        0.836 &         0.844 &         0.973 &           0.772 &          0.987 &     0.978 &       0.715 &      0.978 &      0.972 &        0.725 &       0.974 \\
1080ti\_256                         &     0.741 &       1.000 &      0.747 &     0.726 &       0.820 &      0.745 &                         0.681 &                     0.683 &                      0.617 &                      0.667 &                   0.566 &            0.807 &   0.893 &  0.888 &      0.776 &      0.782 &                              0.672 &                            0.669 &                            0.746 &                               0.632 &                               0.625 &                              0.659 &                              0.644 &                              0.679 &  0.777 &  0.737 &  0.735 &        0.771 &       0.753 &        0.764 &         0.788 &         0.701 &           0.812 &          0.733 &     0.731 &       0.996 &      0.738 &      0.726 &        0.998 &       0.740 \\
1080ti\_32                          &     0.971 &       0.747 &      1.000 &     0.951 &       0.799 &      0.974 &                         0.374 &                     0.376 &                      0.509 &                      0.734 &                   0.172 &            0.842 &   0.434 &  0.841 &      0.956 &      0.847 &                              0.676 &                            0.644 &                            0.645 &                               0.594 &                               0.583 &                              0.623 &                              0.608 &                              0.567 &  0.817 &  0.611 &  0.669 &        0.819 &       0.889 &        0.850 &         0.858 &         0.959 &           0.792 &          0.977 &     0.967 &       0.722 &      0.969 &      0.962 &        0.731 &       0.964 \\
2080ti\_1                           &     0.965 &       0.726 &      0.951 &     1.000 &       0.758 &      0.966 &                         0.353 &                     0.356 &                      0.512 &                      0.730 &                   0.168 &            0.826 &   0.405 &  0.809 &      0.939 &      0.814 &                              0.658 &                            0.625 &                            0.635 &                               0.586 &                               0.581 &                              0.597 &                              0.581 &                              0.538 &  0.791 &  0.578 &  0.637 &        0.782 &       0.867 &        0.811 &         0.823 &         0.959 &           0.751 &          0.968 &     0.959 &       0.700 &      0.960 &      0.954 &        0.711 &       0.955 \\
2080ti\_256                         &     0.780 &       0.820 &      0.799 &     0.758 &       1.000 &      0.788 &                         0.553 &                     0.555 &                      0.477 &                      0.655 &                   0.297 &            0.901 &   0.700 &  0.977 &      0.877 &      0.945 &                              0.753 &                            0.739 &                            0.662 &                               0.596 &                               0.554 &                              0.779 &                              0.770 &                              0.755 &  0.881 &  0.877 &  0.892 &        0.975 &       0.858 &        0.948 &         0.983 &         0.747 &           1.000 &          0.801 &     0.781 &       0.811 &      0.787 &      0.776 &        0.816 &       0.792 \\
2080ti\_32                          &     0.981 &       0.745 &      0.974 &     0.966 &       0.788 &      1.000 &                         0.369 &                     0.371 &                      0.519 &                      0.743 &                   0.174 &            0.849 &   0.424 &  0.836 &      0.960 &      0.843 &                              0.677 &                            0.644 &                            0.650 &                               0.598 &                               0.591 &                              0.619 &                              0.603 &                              0.560 &  0.814 &  0.601 &  0.663 &        0.812 &       0.892 &        0.842 &         0.852 &         0.971 &           0.782 &          0.987 &     0.981 &       0.721 &      0.982 &      0.972 &        0.731 &       0.975 \\
d\_cpu\_core\_i7\_7820x\_fp32       &     0.360 &       0.681 &      0.374 &     0.353 &       0.553 &      0.369 &                         1.000 &                     0.997 &                      0.775 &                      0.697 &                   0.843 &            0.521 &   0.745 &  0.615 &      0.437 &      0.505 &                              0.717 &                            0.725 &                            0.814 &                               0.729 &                               0.726 &                              0.728 &                              0.720 &                              0.797 &  0.501 &  0.664 &  0.637 &        0.511 &       0.448 &        0.487 &         0.509 &         0.313 &           0.551 &          0.344 &     0.360 &       0.700 &      0.367 &      0.355 &        0.698 &       0.368 \\
d\_gpu\_gtx\_1080ti\_fp32           &     0.362 &       0.683 &      0.376 &     0.356 &       0.555 &      0.371 &                         0.997 &                     1.000 &                      0.776 &                      0.699 &                   0.843 &            0.522 &   0.746 &  0.616 &      0.438 &      0.507 &                              0.718 &                            0.727 &                            0.816 &                               0.730 &                               0.727 &                              0.729 &                              0.722 &                              0.799 &  0.501 &  0.665 &  0.639 &        0.513 &       0.450 &        0.488 &         0.511 &         0.315 &           0.552 &          0.346 &     0.362 &       0.701 &      0.369 &      0.356 &        0.699 &       0.370 \\
e\_gpu\_jetson\_nano\_fp16          &     0.514 &       0.617 &      0.509 &     0.512 &       0.477 &      0.519 &                         0.775 &                     0.776 &                      1.000 &                      0.875 &                   0.792 &            0.542 &   0.556 &  0.593 &      0.543 &      0.506 &                              0.791 &                            0.776 &                            0.900 &                               0.874 &                               0.906 &                              0.731 &                              0.720 &                              0.774 &  0.516 &  0.561 &  0.575 &        0.485 &       0.530 &        0.491 &         0.500 &         0.469 &           0.473 &          0.476 &     0.515 &       0.631 &      0.517 &      0.510 &        0.634 &       0.513 \\
e\_gpu\_jetson\_nano\_fp32          &     0.739 &       0.667 &      0.734 &     0.730 &       0.655 &      0.743 &                         0.697 &                     0.699 &                      0.875 &                      1.000 &                   0.575 &            0.715 &   0.490 &  0.739 &      0.765 &      0.697 &                              0.907 &                            0.873 &                            0.939 &                               0.909 &                               0.919 &                              0.843 &                              0.828 &                              0.836 &  0.681 &  0.658 &  0.698 &        0.675 &       0.726 &        0.692 &         0.702 &         0.703 &           0.651 &          0.721 &     0.741 &       0.668 &      0.742 &      0.735 &        0.674 &       0.739 \\
e\_tpu\_edge\_tpu\_int8             &     0.167 &       0.566 &      0.172 &     0.168 &       0.297 &      0.174 &                         0.843 &                     0.843 &                      0.792 &                      0.575 &                   1.000 &            0.315 &   0.699 &  0.408 &      0.221 &      0.268 &                              0.551 &                            0.564 &                            0.736 &                               0.677 &                               0.704 &                              0.539 &                              0.530 &                              0.642 &  0.299 &  0.464 &  0.425 &        0.261 &       0.246 &        0.243 &         0.256 &         0.113 &           0.294 &          0.127 &     0.166 &       0.595 &      0.171 &      0.163 &        0.591 &       0.170 \\
essential\_ph\_1                    &     0.842 &       0.807 &      0.842 &     0.826 &       0.901 &      0.849 &                         0.521 &                     0.522 &                      0.542 &                      0.715 &                   0.315 &            1.000 &   0.624 &  0.924 &      0.898 &      0.888 &                              0.738 &                            0.716 &                            0.692 &                               0.636 &                               0.612 &                              0.725 &                              0.714 &                              0.701 &  0.856 &  0.779 &  0.808 &        0.896 &       0.880 &        0.892 &         0.917 &         0.811 &           0.897 &          0.851 &     0.845 &       0.797 &      0.848 &      0.836 &        0.803 &       0.847 \\
eyeriss                             &     0.415 &       0.893 &      0.434 &     0.405 &       0.700 &      0.424 &                         0.745 &                     0.746 &                      0.556 &                      0.490 &                   0.699 &            0.624 &   1.000 &  0.753 &      0.503 &      0.609 &                              0.561 &                            0.577 &                            0.649 &                               0.545 &                               0.532 &                              0.591 &                              0.584 &                              0.659 &  0.609 &  0.722 &  0.679 &        0.625 &       0.521 &        0.586 &         0.618 &         0.362 &           0.695 &          0.403 &     0.409 &       0.909 &      0.418 &      0.405 &        0.906 &       0.423 \\
fpga                                &     0.828 &       0.888 &      0.841 &     0.809 &       0.977 &      0.836 &                         0.615 &                     0.616 &                      0.593 &                      0.739 &                   0.408 &            0.924 &   0.753 &  1.000 &      0.912 &      0.945 &                              0.795 &                            0.778 &                            0.749 &                               0.684 &                               0.656 &                              0.798 &                              0.786 &                              0.786 &  0.898 &  0.872 &  0.890 &        0.959 &       0.888 &        0.943 &         0.974 &         0.789 &           0.974 &          0.836 &     0.829 &       0.882 &      0.835 &      0.822 &        0.887 &       0.837 \\
gold\_6226                          &     0.958 &       0.776 &      0.956 &     0.939 &       0.877 &      0.960 &                         0.437 &                     0.438 &                      0.543 &                      0.765 &                   0.221 &            0.898 &   0.503 &  0.912 &      1.000 &      0.906 &                              0.742 &                            0.709 &                            0.690 &                               0.643 &                               0.626 &                              0.703 &                              0.688 &                              0.654 &  0.869 &  0.711 &  0.763 &        0.894 &       0.920 &        0.912 &         0.927 &         0.936 &           0.872 &          0.965 &     0.956 &       0.757 &      0.958 &      0.950 &        0.766 &       0.957 \\
gold\_6240                          &     0.831 &       0.782 &      0.847 &     0.814 &       0.945 &      0.843 &                         0.505 &                     0.507 &                      0.506 &                      0.697 &                   0.268 &            0.888 &   0.609 &  0.945 &      0.906 &      1.000 &                              0.751 &                            0.729 &                            0.668 &                               0.617 &                               0.585 &                              0.752 &                              0.741 &                              0.718 &  0.863 &  0.819 &  0.844 &        0.941 &       0.877 &        0.930 &         0.958 &         0.800 &           0.944 &          0.850 &     0.836 &       0.770 &      0.840 &      0.830 &        0.776 &       0.848 \\
m\_cpu\_sd\_450\_cortex\_a53\_int8  &     0.670 &       0.672 &      0.676 &     0.658 &       0.753 &      0.677 &                         0.717 &                     0.718 &                      0.791 &                      0.907 &                   0.551 &            0.738 &   0.561 &  0.795 &      0.742 &      0.751 &                              1.000 &                            0.905 &                            0.898 &                               0.860 &                               0.849 &                              0.981 &                              0.901 &                              0.913 &  0.713 &  0.770 &  0.794 &        0.756 &       0.721 &        0.750 &         0.770 &         0.630 &           0.752 &          0.663 &     0.674 &       0.676 &      0.677 &      0.669 &        0.680 &       0.678 \\
m\_cpu\_sd\_675\_kryo\_460\_int8    &     0.636 &       0.669 &      0.644 &     0.625 &       0.739 &      0.644 &                         0.725 &                     0.727 &                      0.776 &                      0.873 &                   0.564 &            0.716 &   0.577 &  0.778 &      0.709 &      0.729 &                              0.905 &                            1.000 &                            0.877 &                               0.909 &                               0.821 &                              0.895 &                              0.971 &                              0.894 &  0.693 &  0.771 &  0.789 &        0.739 &       0.693 &        0.727 &         0.748 &         0.596 &           0.740 &          0.630 &     0.639 &       0.673 &      0.643 &      0.634 &        0.677 &       0.643 \\
m\_cpu\_sd\_855\_kryo\_485\_int8    &     0.645 &       0.746 &      0.645 &     0.635 &       0.662 &      0.650 &                         0.814 &                     0.816 &                      0.900 &                      0.939 &                   0.736 &            0.692 &   0.649 &  0.749 &      0.690 &      0.668 &                              0.898 &                            0.877 &                            1.000 &                               0.912 &                               0.920 &                              0.858 &                              0.841 &                              0.891 &  0.663 &  0.708 &  0.723 &        0.657 &       0.669 &        0.659 &         0.673 &         0.600 &           0.658 &          0.623 &     0.645 &       0.753 &      0.649 &      0.640 &        0.757 &       0.647 \\
m\_dsp\_sd\_675\_hexagon\_685\_int8 &     0.593 &       0.632 &      0.594 &     0.586 &       0.596 &      0.598 &                         0.729 &                     0.730 &                      0.874 &                      0.909 &                   0.677 &            0.636 &   0.545 &  0.684 &      0.643 &      0.617 &                              0.860 &                            0.909 &                            0.912 &                               1.000 &                               0.922 &                              0.813 &                              0.874 &                              0.839 &  0.609 &  0.658 &  0.680 &        0.607 &       0.625 &        0.609 &         0.622 &         0.547 &           0.593 &          0.568 &     0.597 &       0.643 &      0.599 &      0.591 &        0.646 &       0.596 \\
m\_dsp\_sd\_855\_hexagon\_690\_int8 &     0.587 &       0.625 &      0.583 &     0.581 &       0.554 &      0.591 &                         0.726 &                     0.727 &                      0.906 &                      0.919 &                   0.704 &            0.612 &   0.532 &  0.656 &      0.626 &      0.585 &                              0.849 &                            0.821 &                            0.920 &                               0.922 &                               1.000 &                              0.791 &                              0.779 &                              0.822 &  0.585 &  0.620 &  0.642 &        0.569 &       0.606 &        0.576 &         0.586 &         0.541 &           0.550 &          0.556 &     0.590 &       0.636 &      0.592 &      0.585 &        0.640 &       0.589 \\
m\_gpu\_sd\_450\_adreno\_506\_int8  &     0.610 &       0.659 &      0.623 &     0.597 &       0.779 &      0.619 &                         0.728 &                     0.729 &                      0.731 &                      0.843 &                   0.539 &            0.725 &   0.591 &  0.798 &      0.703 &      0.752 &                              0.981 &                            0.895 &                            0.858 &                               0.813 &                               0.791 &                              1.000 &                              0.916 &                              0.933 &  0.705 &  0.804 &  0.817 &        0.772 &       0.692 &        0.753 &         0.778 &         0.569 &           0.781 &          0.611 &     0.615 &       0.665 &      0.619 &      0.611 &        0.668 &       0.622 \\
m\_gpu\_sd\_675\_adreno\_612\_int8  &     0.594 &       0.644 &      0.608 &     0.581 &       0.770 &      0.603 &                         0.720 &                     0.722 &                      0.720 &                      0.828 &                   0.530 &            0.714 &   0.584 &  0.786 &      0.688 &      0.741 &                              0.901 &                            0.971 &                            0.841 &                               0.874 &                               0.779 &                              0.916 &                              1.000 &                              0.919 &  0.695 &  0.804 &  0.816 &        0.764 &       0.679 &        0.742 &         0.768 &         0.554 &           0.772 &          0.595 &     0.600 &       0.650 &      0.604 &      0.594 &        0.653 &       0.605 \\
m\_gpu\_sd\_855\_adreno\_640\_int8  &     0.551 &       0.679 &      0.567 &     0.538 &       0.755 &      0.560 &                         0.797 &                     0.799 &                      0.774 &                      0.836 &                   0.642 &            0.701 &   0.659 &  0.786 &      0.654 &      0.718 &                              0.913 &                            0.894 &                            0.891 &                               0.839 &                               0.822 &                              0.933 &                              0.919 &                              1.000 &  0.684 &  0.819 &  0.820 &        0.741 &       0.653 &        0.717 &         0.743 &         0.504 &           0.757 &          0.547 &     0.557 &       0.691 &      0.562 &      0.551 &        0.693 &       0.564 \\
pixel2                              &     0.807 &       0.777 &      0.817 &     0.791 &       0.881 &      0.814 &                         0.501 &                     0.501 &                      0.516 &                      0.681 &                   0.299 &            0.856 &   0.609 &  0.898 &      0.869 &      0.863 &                              0.713 &                            0.693 &                            0.663 &                               0.609 &                               0.585 &                              0.705 &                              0.695 &                              0.684 &  1.000 &  0.761 &  0.787 &        0.874 &       0.832 &        0.873 &         0.894 &         0.775 &           0.878 &          0.817 &     0.809 &       0.767 &      0.813 &      0.801 &        0.773 &       0.816 \\
pixel3                              &     0.591 &       0.737 &      0.611 &     0.578 &       0.877 &      0.601 &                         0.664 &                     0.665 &                      0.561 &                      0.658 &                   0.464 &            0.779 &   0.722 &  0.872 &      0.711 &      0.819 &                              0.770 &                            0.771 &                            0.708 &                               0.658 &                               0.620 &                              0.804 &                              0.804 &                              0.819 &  0.761 &  1.000 &  0.967 &        0.849 &       0.717 &        0.814 &         0.847 &         0.547 &           0.878 &          0.599 &     0.591 &       0.742 &      0.598 &      0.589 &        0.744 &       0.607 \\
raspi4                              &     0.654 &       0.735 &      0.669 &     0.637 &       0.892 &      0.663 &                         0.637 &                     0.639 &                      0.575 &                      0.698 &                   0.425 &            0.808 &   0.679 &  0.890 &      0.763 &      0.844 &                              0.794 &                            0.789 &                            0.723 &                               0.680 &                               0.642 &                              0.817 &                              0.816 &                              0.820 &  0.787 &  0.967 &  1.000 &        0.875 &       0.758 &        0.844 &         0.878 &         0.609 &           0.893 &          0.663 &     0.659 &       0.736 &      0.664 &      0.652 &        0.739 &       0.668 \\
samsung\_a50                        &     0.804 &       0.771 &      0.819 &     0.782 &       0.975 &      0.812 &                         0.511 &                     0.513 &                      0.485 &                      0.675 &                   0.261 &            0.896 &   0.625 &  0.959 &      0.894 &      0.941 &                              0.756 &                            0.739 &                            0.657 &                               0.607 &                               0.569 &                              0.772 &                              0.764 &                              0.741 &  0.874 &  0.849 &  0.875 &        1.000 &       0.872 &        0.946 &         0.978 &         0.773 &           0.975 &          0.824 &     0.808 &       0.762 &      0.813 &      0.801 &        0.767 &       0.816 \\
samsung\_s7                         &     0.887 &       0.753 &      0.889 &     0.867 &       0.858 &      0.892 &                         0.448 &                     0.450 &                      0.530 &                      0.726 &                   0.246 &            0.880 &   0.521 &  0.888 &      0.920 &      0.877 &                              0.721 &                            0.693 &                            0.669 &                               0.625 &                               0.606 &                              0.692 &                              0.679 &                              0.653 &  0.832 &  0.717 &  0.758 &        0.872 &       1.000 &        0.876 &         0.896 &         0.861 &           0.854 &          0.894 &     0.884 &       0.737 &      0.887 &      0.881 &        0.746 &       0.888 \\
silver\_4114                        &     0.836 &       0.764 &      0.850 &     0.811 &       0.948 &      0.842 &                         0.487 &                     0.488 &                      0.491 &                      0.692 &                   0.243 &            0.892 &   0.586 &  0.943 &      0.912 &      0.930 &                              0.750 &                            0.727 &                            0.659 &                               0.609 &                               0.576 &                              0.753 &                              0.742 &                              0.717 &  0.873 &  0.814 &  0.844 &        0.946 &       0.876 &        1.000 &         0.964 &         0.806 &           0.947 &          0.853 &     0.836 &       0.751 &      0.841 &      0.834 &        0.758 &       0.844 \\
silver\_4210r                       &     0.844 &       0.788 &      0.858 &     0.823 &       0.983 &      0.852 &                         0.509 &                     0.511 &                      0.500 &                      0.702 &                   0.256 &            0.917 &   0.618 &  0.974 &      0.927 &      0.958 &                              0.770 &                            0.748 &                            0.673 &                               0.622 &                               0.586 &                              0.778 &                              0.768 &                              0.743 &  0.894 &  0.847 &  0.878 &        0.978 &       0.896 &        0.964 &         1.000 &         0.815 &           0.982 &          0.863 &     0.847 &       0.776 &      0.852 &      0.841 &        0.782 &       0.854 \\
titan\_rtx\_1                       &     0.973 &       0.701 &      0.959 &     0.959 &       0.747 &      0.971 &                         0.313 &                     0.315 &                      0.469 &                      0.703 &                   0.113 &            0.811 &   0.362 &  0.789 &      0.936 &      0.800 &                              0.630 &                            0.596 &                            0.600 &                               0.547 &                               0.541 &                              0.569 &                              0.554 &                              0.504 &  0.775 &  0.547 &  0.609 &        0.773 &       0.861 &        0.806 &         0.815 &         1.000 &           0.740 &          0.980 &     0.965 &       0.672 &      0.965 &      0.962 &        0.683 &       0.962 \\
titan\_rtx\_256                     &     0.772 &       0.812 &      0.792 &     0.751 &       1.000 &      0.782 &                         0.551 &                     0.552 &                      0.473 &                      0.651 &                   0.294 &            0.897 &   0.695 &  0.974 &      0.872 &      0.944 &                              0.752 &                            0.740 &                            0.658 &                               0.593 &                               0.550 &                              0.781 &                              0.772 &                              0.757 &  0.878 &  0.878 &  0.893 &        0.975 &       0.854 &        0.947 &         0.982 &         0.740 &           1.000 &          0.794 &     0.774 &       0.803 &      0.780 &      0.769 &        0.808 &       0.785 \\
titan\_rtx\_32                      &     0.987 &       0.733 &      0.977 &     0.968 &       0.801 &      0.987 &                         0.344 &                     0.346 &                      0.476 &                      0.721 &                   0.127 &            0.851 &   0.403 &  0.836 &      0.965 &      0.850 &                              0.663 &                            0.630 &                            0.623 &                               0.568 &                               0.556 &                              0.611 &                              0.595 &                              0.547 &  0.817 &  0.599 &  0.663 &        0.824 &       0.894 &        0.853 &         0.863 &         0.980 &           0.794 &          1.000 &     0.982 &       0.705 &      0.983 &      0.976 &        0.715 &       0.979 \\
titanx\_1                           &     0.978 &       0.731 &      0.967 &     0.959 &       0.781 &      0.981 &                         0.360 &                     0.362 &                      0.515 &                      0.741 &                   0.166 &            0.845 &   0.409 &  0.829 &      0.956 &      0.836 &                              0.674 &                            0.639 &                            0.645 &                               0.597 &                               0.590 &                              0.615 &                              0.600 &                              0.557 &  0.809 &  0.591 &  0.659 &        0.808 &       0.884 &        0.836 &         0.847 &         0.965 &           0.774 &          0.982 &     1.000 &       0.707 &      0.981 &      0.970 &        0.716 &       0.971 \\
titanx\_256                         &     0.715 &       0.996 &      0.722 &     0.700 &       0.811 &      0.721 &                         0.700 &                     0.701 &                      0.631 &                      0.668 &                   0.595 &            0.797 &   0.909 &  0.882 &      0.757 &      0.770 &                              0.676 &                            0.673 &                            0.753 &                               0.643 &                               0.636 &                              0.665 &                              0.650 &                              0.691 &  0.767 &  0.742 &  0.736 &        0.762 &       0.737 &        0.751 &         0.776 &         0.672 &           0.803 &          0.705 &     0.707 &       1.000 &      0.714 &      0.701 &        0.998 &       0.715 \\
titanx\_32                          &     0.978 &       0.738 &      0.969 &     0.960 &       0.787 &      0.982 &                         0.367 &                     0.369 &                      0.517 &                      0.742 &                   0.171 &            0.848 &   0.418 &  0.835 &      0.958 &      0.840 &                              0.677 &                            0.643 &                            0.649 &                               0.599 &                               0.592 &                              0.619 &                              0.604 &                              0.562 &  0.813 &  0.598 &  0.664 &        0.813 &       0.887 &        0.841 &         0.852 &         0.965 &           0.780 &          0.983 &     0.981 &       0.714 &      1.000 &      0.969 &        0.723 &       0.972 \\
titanxp\_1                          &     0.972 &       0.726 &      0.962 &     0.954 &       0.776 &      0.972 &                         0.355 &                     0.356 &                      0.510 &                      0.735 &                   0.163 &            0.836 &   0.405 &  0.822 &      0.950 &      0.830 &                              0.669 &                            0.634 &                            0.640 &                               0.591 &                               0.585 &                              0.611 &                              0.594 &                              0.551 &  0.801 &  0.589 &  0.652 &        0.801 &       0.881 &        0.834 &         0.841 &         0.962 &           0.769 &          0.976 &     0.970 &       0.701 &      0.969 &      1.000 &        0.711 &       0.965 \\
titanxp\_256                        &     0.725 &       0.998 &      0.731 &     0.711 &       0.816 &      0.731 &                         0.698 &                     0.699 &                      0.634 &                      0.674 &                   0.591 &            0.803 &   0.906 &  0.887 &      0.766 &      0.776 &                              0.680 &                            0.677 &                            0.757 &                               0.646 &                               0.640 &                              0.668 &                              0.653 &                              0.693 &  0.773 &  0.744 &  0.739 &        0.767 &       0.746 &        0.758 &         0.782 &         0.683 &           0.808 &          0.715 &     0.716 &       0.998 &      0.723 &      0.711 &        1.000 &       0.725 \\
titanxp\_32                         &     0.974 &       0.740 &      0.964 &     0.955 &       0.792 &      0.975 &                         0.368 &                     0.370 &                      0.513 &                      0.739 &                   0.170 &            0.847 &   0.423 &  0.837 &      0.957 &      0.848 &                              0.678 &                            0.643 &                            0.647 &                               0.596 &                               0.589 &                              0.622 &                              0.605 &                              0.564 &  0.816 &  0.607 &  0.668 &        0.816 &       0.888 &        0.844 &         0.854 &         0.962 &           0.785 &          0.979 &     0.971 &       0.715 &      0.972 &      0.965 &        0.725 &       1.000 \\
\bottomrule
\end{tabular}


    
}
\caption{Device correlations}
\label{tab:alldevcor}
\end{table*}

==> backup.tex <==

% \centering
% \resizebox{0.8\linewidth}{!}{%
% %\begin{adjustbox}{width=0.8\columnwidth}
% \begin{tabular}{@{}l|c|c|c|c@{}}
% \toprule
% \multicolumn{1}{l}{\textbf{Search space}} & \multicolumn{1}{c}{\textbf{Tasks}} & 
% \multicolumn{1}{c}{\textbf{Num.\ ZC proxies}} & 
% \multicolumn{1}{c}{\textbf{Num.\ architectures}} &
% \multicolumn{1}{c}{\textbf{Total ZC proxy evaluations}} \\
% \midrule
% NAS-Bench-101 & 1 & 13 & 423\,625 & 5\,507\,125 \\
% NAS-Bench-201 & 1 & 13 & 15\,625 & 203\,125 \\
% DARTS                                   & 1 & 13 & 5000 & 65000 \\
% ENAS                                    & 1 & 13 & 4999 & 64987 \\
% PNAS                                    & 1 & 13 & 4999 & 64987 \\
% NASNet                                  & 1 & 13 & 4846 & 62998 \\
% AmoebaNet                               & 1 & 13 & 4983 & 64779 \\
% DARTS$_{FixWD}$                         & 1 & 13 & 5000 & 65000 \\
% DARTS$_{LRWD}$                          & 1 & 13 & 5000 & 65000 \\
% ENAS$_{FixWD}$                          & 1 & 13 & 5000 & 65000 \\
% PNAS$_{FixWD}$                          & 1 & 13 & 4559 & 59267 \\
% TransNASBench-101 Micro& 7 & 12 & 4096 & 344\,064\\
% \textbf{Total} & 18 & 13 & 512\,308 & 6\,631\,332 \\
% % 344064 + 65000 + 64987 + 64987 + 62998 + 64779 + 65000 + 65000 + 65000 + 59267 + 203125 + 5507125
% \bottomrule
% \end{tabular}%
% }
% \caption{Overview of ZC proxy evaluations we use. ZCP for TransNASBench-101 Micro and NASBench201 are borrowed from \cite{nasbenchsuitezero}. Additionally, we utilize CATE and Arch2Vec representations for these spaces as well.}
% \label{tab:zcp_details}
% \end{table*}
% \begin{table}[t!]
%   \centering
% \caption{We study the impact of design choices on the performance of predictors on three FBNet device sets. \yash{try to regen or add F3.}}\vspace{2mm}
% \label{table:design_components}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{lccc}
% \toprule
%                               & F1 & F2 & F4 \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-4} \addlinespace[0.5ex]
% GIN                            & $0.772_{0.071}$ & $0.713_{0.094}$ & $0.875_{0.023}$ \\
% (+ HWInit)                     & $0.805_{0.046}$ & $0.830_{0.022}$ & $0.887_{0.021}$ \\
% (+ Op$_{HW}$)                  & \bB$0.842_{0.028}$ & \bR$0.842_{0.012}$ & $0.906_{0.008}$ \\
% (+ Sampler)                    & $0.844_{0.020}$ & $0.840_{0.008}$ & \bB$0.909_{0.005}$ \\
% (+ Supp. Encoding)             & \bR$0.905_{0.011}$ & \bB$0.841_{0.011}$ & \bR$0.942_{0.007}$ \\
% \bottomrule

% \end{tabular}%
% }
% \end{table}


% \begin{table}[t!]
%   \centering
% \caption{We study the impact of design choices on the performance of predictors.}\vspace{2mm}
% \label{table:design_components_nb201}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
%                         & N1 & N2 & N3 & N4 \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-5} \addlinespace[0.5ex]
% GIN                    & $0.938_{0.034}$ & $0.781_{0.084}$  & $0.907_{0.019}$ & $0.922_{0.021}$ \\
% (+ HWInit)             & $0.938_{0.031}$ & $0.776_{0.039}$  & $0.887_{0.087}$ & $0.898_{0.046}$ \\
% (+ Op$_{HW}$)          & \bB$0.949_{0.017}$ & \bR$0.821_{0.045}$  & \bR$0.938_{0.021}$ \bB& $0.955_{0.015}$ \\
% (+ Sampler)            & \bR$0.962_{0.012}$ & $0.803_{0.067}$  & $0.920_{0.034}$ & \bR$0.961_{0.007}$ \\
% (+ Supp. Encoding)     & $0.936_{0.033}$ & \bB$0.812_{0.059}$  & \bB$0.930_{0.028}$ & $0.940_{0.017}$ \\
% \bottomrule

% \end{tabular}%
% }
% \end{table}


% \begin{table}[t!]
%        \centering
%      \caption{Cosine based selection for samplers with vector encodings outperforms kMeans.}\vspace{2mm}
%      \label{table:kmeans_cosine}
%        \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccccccccc}
% \toprule
%        & \multicolumn{4}{c}{10 Samples}            & \multicolumn{4}{c}{20 Samples}            \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \addlinespace[0.5ex]
% NB201  & ZCP      & Arch2Vec & CATE     & CAZ      & ZCP      & Arch2Vec & CATE     & CAZ      \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \addlinespace[0.5ex]
% Cosine & \bR$0.948$ & \bR$0.949$ & \bR$0.933$ & \bR$0.951$ & \bR$0.963$  & \bR$0.960$ & \bR$0.952$ & \bR$0.960$ \\
% Kmeans & $0.729$ & $0.670$ & $0.826$ & $0.892$ & $0.786$ & $0.680$  & $0.885$  & $0.948$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \addlinespace[0.5ex]
% FBNet  & ZCP      & Arch2Vec & CATE     & CAZ      & ZCP      & Arch2Vec & CATE     & CAZ      \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \addlinespace[0.5ex]
% Cosine & \bR$0.822$ & \bR$0.803$ & \bR$0.805$ & \bR$0.788$ & \bR$0.845$ & \bR$0.839$ & \bR$0.828$ & \bR$0.852$ \\
% Kmeans & $0.412$ & $0.657$ & NaN      & $0.718$ & $0.818$  & $0.812$ & NaN      & $0.835$ \\\bottomrule
% \end{tabular}%
% }
% \end{table}

% \section{Latency Predictor Design}
% \label{sec:latpreddesign}
% \begin{table*}[t!]
%     \centering
%   \caption{Using operation-wise hardware embedding to capture operation interactions improve performance. 20 samples used for transfer.}\vspace{2mm}
%   \label{table:hw_mlp_hwinit}
%     \resizebox{\linewidth}{!}{%
%   \centering
% \begin{tabular}{ccccccccccccc}
% \toprule
% Opwise HWEmb    &       ND  &       N1  &       N2  &       N3  &       N4   &      NA  &       FD  &       F1  &       F2  &       F3  &       F4  &       FA \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]
% \ding{51} &       \bR$0.806_{0.038}$ & \bR$0.719_{0.050}$ & \bR$0.795_{0.034}$ & \bR$0.704_{0.058}$ & $0.753_{0.052}$ & \bR$0.664_{0.059}$ & \bR$0.845_{0.009}$ & \bR$0.757_{0.048}$ & \bR$0.769_{0.076}$ & \bR$0.694_{0.076}$ & \bR$0.832_{0.026}$ & \bR$0.628_{0.103}$ \\
% \ding{55}  &       $0.804_{0.026}$ & $0.701_{0.056}$ & $0.763_{0.044}$ & $0.680_{0.042}$ & \bR$0.757_{0.061}$ & $0.660_{0.030}$ & $0.839_{0.010}$ & $0.753_{0.031}$ & $0.745_{0.081}$ & $0.685_{0.085}$ & $0.813_{0.030}$ & $0.566_{0.081}$ \\\cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]

% HWEmb Init    &       ND  &       N1  &       N2  &       N3  &       N4   &      NA  &       FD  &       F1  &       F2  &       F3  &       F4  &       FA \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]
% \ding{51} &       \bR$0.806_{0.038}$ & \bR$0.719_{0.050}$ & \bR$0.795_{0.034}$ & $0.704_{0.058}$ & \bR$0.753_{0.052}$ & \bR$0.664_{0.059}$ & \bR$0.845_{0.009}$ & \bR$0.757_{0.048}$ & \bR$0.769_{0.076}$ & \bR$0.694_{0.076}$ & \bR$0.832_{0.026}$ & \bR$0.628_{0.103}$ \\
% \ding{55} & $0.794_{0.038}$ & $0.701_{0.046}$ & $0.791_{0.036}$ & \bR$0.718_{0.055}$ & $0.750_{0.050}$ & $0.658_{0.080}$ & $0.707_{0.158}$ & $0.609_{0.119}$ & $0.754_{0.064}$ & $0.655_{0.084}$ & $0.659_{0.158}$ & $0.559_{0.118}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

% BRPNAS \cite{brpnas} introduced graph convolutional networks for accuracy and latency prediction, which significantly improves prediction performance compared to multi-layer perceptrons. Recent literature focused on improving the performance of these GCNs for accuracy prediction by introducing residual connections \cite{tagates} in the graph neural network module, as well as an operation embedding update methodology which is independent from predictor training that refines the embedding such that it captures more information about the operations in the network. 

% \begin{table*}[t!]
%   \centering
% \caption{Over three device sets on two NAS spaces, there is a benefit in using supplementary encodings for representing neural networks. CAZ was used as the sampler and 20 samples are fetched for transfer to ensure effective training of baseline predictor.\yash{TABLE REDO UNDER PROGRESS}}\vspace{2mm}
% \label{table:adj_gin_enc_study}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{lllllllllllll}
% \toprule
% Encoding &                ND &                N1 &                N2 &                N3 &                N4 &                NA &                FD &                F1 &                F2 &                F3 &                F4 &                FA \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]
% AdjOp              &  $0.960_{0.010}$ &  $0.737_{0.016}$ &  $0.630_{0.019}$ &  $0.712_{0.020}$ &  $0.733_{0.020}$ &  $0.587_{0.019}$ & $0.797_{0.043}$  &  $0.290_{0.037}$ &\bR$0.678_{0.067}$ &  $0.526_{0.043}$ &  $0.719_{0.037}$ &  $0.477_{0.051}$ \\\cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]

% (+ Arch2Vec) &\bR$0.965_{0.010}$ &  $0.756_{0.031}$ &\bR$0.641_{0.020}$ &  $0.700_{0.048}$ &  $0.722_{0.011}$ &\bR$0.608_{0.033}$ & $0.888_{0.009}$  &  $0.372_{0.033}$ &  $0.641_{0.062}$ &\bR$0.613_{0.048}$ &\bR$0.762_{0.049}$ &\bR$0.556_{0.021}$ \\
% (+ CATE)     &  $0.964_{0.010}$ &  $0.764_{0.030}$ &  $0.637_{0.018}$ &  $0.706_{0.020}$ &  $0.720_{0.013}$ &  $0.604_{0.026}$ &  $0.858_{0.018}$ &  $0.388_{0.036}$ &  $0.578_{0.062}$ &  $0.478_{0.139}$ &  $0.752_{0.025}$ &  $0.516_{0.053}$ \\
% (+ CAZ)      &  $0.962_{0.007}$ &  $0.739_{0.024}$ &  $0.634_{0.016}$ &  $0.692_{0.031}$ &  $0.726_{0.008}$ &  $0.576_{0.013}$ & $0.946_{0.008}$ &\bR$0.479_{0.053}$ &  $0.445_{0.045}$ &  $0.416_{0.057}$ &  $0.723_{0.036}$ &  $0.463_{0.014}$ \\
% (+ ZCP)      &  $0.964_{0.007}$ &\bR$0.759_{0.030}$ &  $0.636_{0.022}$ &\bR$0.708_{0.029}$ &\bR$0.739_{0.018}$ &  $0.596_{0.021}$ &  \bR$0.963_{0.009}$ &  $0.479_{0.045}$ &  $0.490_{0.038}$ &  $0.444_{0.039}$ &  $0.746_{0.035}$ &  $0.484_{0.015}$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[t!]
%   \centering
% \caption{On NB201, GAT outperforms GCN significantly. On FBNet, the difference is less evident on FBNet, we thus use an Ensemble of GCN and GAT. Here, 20 samples are used for transfer.}\vspace{2mm}
% \label{table:gcn_gat_design}
%   \resizebox{0.8\linewidth}{!}{%
% \begin{tabular}{ccccccccc}
% \toprule
% GNN Module & ND & N1 & N2 & N3 & FD & F1 & F2 & F3 \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \addlinespace[0.5ex]
% GCN       & $0.814_{0.026}$ & $0.741_{0.032}$ & \bR$0.802_{0.021}$ & $0.710_{0.042}$ & \bR$0.844_{0.004}$ & $0.740_{0.055}$ & $0.752_{0.076}$ & \bR$0.621_{0.120}$ \\ 
% GAT       & \bR$0.965_{0.005}$ & \bR$0.848_{0.038}$ & $0.612_{0.032}$ & $0.762_{0.039}$ & $0.823_{0.019}$ & \bR$0.749_{0.042}$ & $0.700_{0.114}$ & $0.589_{0.083}$ \\ 
% Ensemble  & $0.965_{0.011}$ & $0.829_{0.046}$ & $0.634_{0.029}$ & \bR$0.789_{0.054}$ & $0.835_{0.007}$ & $0.733_{0.059}$ & \bR$0.766_{0.013}$ & $0.609_{0.106}$ \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table*}
% \begin{enumerate}
%     \item \textbf{[EXP6.2.1]} transfer hwemb, hwemb to mlp (Rows: tick/cross for True/False, Columns: NB201, FBNet; Sub columns: Task 0, 1 (device average with average std)) Table \ref{table:hw_mlp_hwinit}.
%     \item \textbf{[EXP6.2.2]}DGF, GAT, Ensemble (Rows: tasks, Columns NB201, FBNet; Sub columns: DGF, GAT, Ensemble (device average with average std)) Table \ref{table:gcn_gat_design}
% \end{enumerate}
% \begin{algorithm}[tb]
%    \caption{Bubble Sort}
%    \label{alg:example}
% \begin{algorithmic}
%    \STATE {\bfseries Input:} data $x_i$, size $m$
%    \REPEAT
%    \STATE Initialize $noChange = true$.
%    \FOR{$i=1$ {\bfseries to} $m-1$}
%    \IF{$x_i > x_{i+1}$}
%    \STATE Swap $x_i$ and $x_{i+1}$
%    \STATE $noChange = false$
%    \ENDIF
%    \ENDFOR
%    \UNTIL{$noChange$ is $true$}
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% \caption{Example Bipartite Graph Creation and Node Pruning}
% \begin{algorithmic}[1]
% \Require Graph $G$ of negative correlations, integers $m$, $n$
% \Ensure Modified bipartite graph $B$

% \Statex
% \Function{ComputeWeight}{$v$, $B$}
%     \State \Return $\sum_{u \in \text{neighbors of } v} \text{weight of edge }(u, v)$ in $B$
% \EndFunction
% \Statex

% \State Partition $G$ into two sets $bisect\_m$ and $bisect\_n$ using Kernighan-Lin bisection
% \State Initialize $B$ as a bipartite graph with edges between nodes in $bisect\_m$ and $bisect\_n$ weighted by correlations

% \While{number of nodes in the first partition of $B > m$ OR number of nodes in the second partition of $B > n$}
%     \State $left \gets$ first partition of nodes in $B$
%     \State $right \gets$ second partition of nodes in $B$

%     \If{number of nodes in $left > m$}
%         \State For each node $v$ in $left$, compute $w_v = \Call{ComputeWeight}{v, B}$
%         \State Find node $v^*$ with the highest $w_{v^*}$ in $left$
%         \State Remove node $v^*$ from $B$
%     \EndIf

%     \If{number of nodes in $right > n$}
%         \State For each node $v$ in $right$, compute $w_v = \Call{ComputeWeight}{v, B}$
%         \State Find node $v^*$ with the highest $w_{v^*}$ in $right$
%         \State Remove node $v^*$ from $B$
%     \EndIf

% \EndWhile

% \end{algorithmic}
% \end{algorithm}



% \begin{table*}[t!]
%   \centering
% \caption{On the default (D) and adversarial (A) tasks introduced in HELP and MultiPredict, our predictor with the CAZ and CATE sampler works best for NASBench-201 and FBNet respectively. Standard deviations are reported for results we report.}\vspace{2mm}
% \label{table:all_final_results}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccccccccccccccc}
% \toprule
%   & Source & Target             & \multirow{2}{*}{ND} & \multirow{2}{*}{NA} & \multirow{2}{*}{N1} & \multirow{2}{*}{N2} & \multirow{2}{*}{N3} & \multirow{2}{*}{N4} \\
%   & \multicolumn{2}{c}{Samples} &                     &                     &                     &                     &                     &                      \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-9} \addlinespace[0.5ex]
% HELP                & 900 &  20 & $0.948_{0.006}$ & $0.410_{0.037}$ & $0.604_{0.044}$ & $0.509_{0.007}$ & $0.729_{0.027}$ & $0.746_{0.042}$ \\
% MultiPredict        & 900 &  20 & $0.930_{0.012}$ & $0.820_{0.019}$ & $0.970_{0.003}$ & $0.757_{0.045}$ & $0.947_{0.012}$ & $0.952_{0.011}$ \\
%             Ours    & 25  &  20 & \bR$0.959_{0.007}$ & \bR$0.893_{0.036}$ & \bR$0.967_{0.007}$ & \bR$0.857_{0.029}$ & \bR$0.962_{0.008}$ & \bR$0.959_{0.012}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-9} \addlinespace[0.5ex]
%             & &                 & {FD}                & {FA}                & {F1}                & {F2}                & {F3}                 & {F4} \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-9} \addlinespace[0.5ex]
% HELP                & 4000 &  20 & \bR$0.965_{0.001}$ & $0.406_{0.007}$ & \bR$0.793_{0.028}$ & $0.543_{0.036}$ & $0.413_{0.015}$ & \bR$0.799_{0.004}$   \\
% MultiPredict        & 4000 &  20 & $0.944_{0.012}$ & $0.4701_{0.0636}$ & $0.756_{0.026}$ & $0.567_{0.075}$ & $0.434_{0.040}$ & $0.763_{0.011}$    \\
%             Ours    & 800  &  20 & $0.729_{0.070}$ & \bR$0.507_{0.122}$  & $0.704_{0.059}$ & \bR$0.829_{0.034}$ & \bR$0.831_{0.054}$ & $0.698_{0.091}$\\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


% Contributions:
% \begin{itemize}
%     \item \textbf{Standardized evaluation of latency predictors:} We propose an unbiased method for generating training and testing device sets to fairly evaluate predictor performance. We provide 6 train-test device sets over two NAS distinct spaces and evaluate latency predictors on the spaces.
%     \item \textbf{Latency predictor architecture:} We propose a methodology to encode lower-level interactions between operations in a neural network with graph neural networks to build a novel latency predictor that outperforms prior methods, demonstrating a \red{10$\times$} improvement in prediction accuracy.
%     \item \textbf{Leveraging neural network encodings:} We utilize unsupervised representation learning based and property based neural network encodings to figure out the right neural network architectures to sample for devices to reduce variance.
% \end{itemize}
    % \item \textbf{}
    % \item \textbf{}
    % \item State of the art latency predictor with transfer learning support.
    % \item Demonstrating applicability of algorithm on micro and macro cell spaces (NB201 and FBNet).
    % \item Leveraging supplemental encodings to improve latency predictor performance. 
    % \item Generate encodings for FBNet and NASBench-201 and leverage them to create better network samplers.
    % \item Designing difficult problems for effective evaluation of existing and our methodology. 

% center around: Discuss: methodology issue (device selection etc), sampling (variance issue), micro vs macro architectural: structure contributions in this manner?


% \begin{table*}[t!]
%     \centering
%   \caption{Over three device sets on two NAS spaces, there is a benefit in using supplementary encodings for training-transfer sample selection. Latency (Oracle) is not highlighted as it uses ground truth latency information over the entire data-set to select networks. Only 5 samples are used for transfer to effectively test sampler. \yash{added N0, F0 N4, F4, N5, F5 in table below}}\vspace{2mm}
%   \label{table:sampler_study}
%     \resizebox{.8\linewidth}{!}{%
%   \begin{tabular}{lccccccc}
%   \toprule
%   Sampler &                N1 &                N2 &                N3&                F1 &                F2 &                F3 \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \addlinespace[0.5ex]
%   Latency (Oracle)    &  $0.799_{0.094}$  &   $0.663_{0.026}$ &   $0.738_{0.097}$ &   $0.689_{0.130}$ &   $0.718_{0.080}$ &   $0.693_{0.050}$ \\
%   Random              &  $0.777_{0.087}$  &   $0.644_{0.038}$ &   $0.742_{0.069}$ &\bR$0.715_{0.095}$ &   $0.702_{0.075}$ &\bB$0.665_{0.085}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \addlinespace[0.5ex] 
%   Params              &  $0.782_{0.090}$  &\bR$0.654_{0.033}$ &   $0.732_{0.081}$ &   $0.689_{0.130}$ &\bB$0.713_{0.087}$ &   $0.659_{0.095}$ \\
%   CATE                &\bB$0.799_{0.030}$ &   $0.649_{0.028}$ &\bR$0.824_{0.026}$ &   $0.145_{0.090}$ &   $0.489_{0.115}$ &   $0.276_{0.169}$ \\
%   Arch2Vec            &  $0.719_{0.068}$  &\bB$0.653_{0.028}$ &   $0.711_{0.062}$ &   $0.671_{0.067}$ &   $0.590_{0.088}$ &   $0.633_{0.072}$ \\
%   ZCP                 &\bR$0.825_{0.022}$ &   $0.626_{0.027}$ &   $0.729_{0.078}$ &\bB$0.694_{0.040}$ &   $0.570_{0.127}$ &   $0.625_{0.050}$ \\
%   CAZ                 &  $0.788_{0.088}$  &   $0.641_{0.024}$ &\bB$0.759_{0.041}$ &   $0.629_{0.138}$ &\bR$0.790_{0.040}$ &\bR$0.671_{0.055}$ \\
%   \bottomrule
%   \end{tabular}
%   }
%   \end{table*}


% \begin{table*}[t!]
%     \centering
%   \caption{Over three device sets on two NAS spaces, there is a benefit in using supplementary encodings for training-transfer sample selection. Latency (Oracle) is not highlighted as it uses ground truth latency information over the entire data-set to select networks. Only 5 samples are used for transfer to effectively test sampler.}\vspace{2mm}
%   \label{table:sampler_study}
%     \resizebox{\linewidth}{!}{%
% \begin{tabular}{lllllllllllll}
% \toprule
% Sampler &                ND &                N1 &                N2 &                N3 &                N4 &                NA & FD &                F1 &                F2 &                F3 &                F4 &                FA \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]
% Random              &  $0.897_{0.057}$ &  $0.777_{0.087}$ &  $0.644_{0.038}$ &  $0.742_{0.069}$ &  $0.805_{0.134}$ &  $0.588_{0.094}$ &  $0.742_{0.047}$ &  \bR$0.715_{0.095}$ &  $0.702_{0.075}$ &  $0.665_{0.085}$ &  $0.730_{0.167}$ &  $0.442_{0.113}$ \\
% Latency (Oracle)    &  $0.907_{0.053}$ &  $0.799_{0.094}$ &  $0.663_{0.026}$ &  $0.738_{0.097}$ &  $0.848_{0.093}$ &  $0.590_{0.105}$ &  $0.732_{0.091}$ &  $0.689_{0.130}$ &  $0.718_{0.080}$ &  $0.693_{0.050}$ &  $0.807_{0.057}$ &  $0.481_{0.140}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]
% Params              &  \bR$0.929_{0.038}$ &  $0.782_{0.090}$ &  \bR$0.654_{0.033}$ &  $0.732_{0.081}$ &  $0.795_{0.139}$ &  $0.604_{0.094}$ &  $0.735_{0.048}$ &  $0.689_{0.130}$ &  $0.713_{0.087}$ &  $0.659_{0.095}$ &  $0.735_{0.160}$ &  \bR$0.521_{0.123}$ \\
% Arch2Vec            &  $0.918_{0.032}$ &  $0.719_{0.068}$ &  $0.653_{0.028}$ &  $0.711_{0.062}$ &  $0.864_{0.118}$ &  $0.528_{0.084}$ &  $0.694_{0.090}$ &  $0.671_{0.067}$ &  $0.590_{0.088}$ &  $0.633_{0.072}$ &  $0.676_{0.131}$ &  $0.455_{0.085}$ \\
% CATE                &  $0.920_{0.012}$ &  $0.799_{0.030}$ &  $0.649_{0.028}$ &  \bR$0.824_{0.026}$ &  $0.770_{0.027}$ &  $0.585_{0.021}$ &  $0.416_{0.123}$ &  $0.145_{0.090}$ &  $0.489_{0.115}$ &  $0.276_{0.169}$ &  $0.302_{0.091}$ &  $0.074_{0.066}$ \\
% ZCP                 &  $0.920_{0.016}$ &  \bR$0.825_{0.022}$ &  $0.626_{0.027}$ &  $0.729_{0.078}$ &  \bR$0.860_{0.094}$ &  $0.608_{0.043}$ &  $0.620_{0.044}$ &  $0.694_{0.040}$ &  $0.570_{0.127}$ &  $0.625_{0.050}$ &  $0.673_{0.129}$ &  $0.434_{0.045}$ \\
% CAZ                 &  $0.932_{0.024}$ &  $0.788_{0.088}$ &  $0.641_{0.024}$ &  $0.759_{0.041}$ &  $0.685_{0.113}$ &  \bR$0.638_{0.065}$ &  \bR$0.751_{0.058}$ &  $0.629_{0.138}$ &  \bR$0.790_{0.040}$ &  \bR$0.671_{0.055}$ &  \bR$0.777_{0.068}$ &  $0.400_{0.091}$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[t!]
%   \centering
% \caption{Over three device sets on two NAS spaces, there is a benefit in using supplementary encodings for representing neural networks. CAZ was used as the sampler and 20 samples are fetched for transfer to ensure effective training of baseline predictor.}\vspace{2mm}
% \label{table:adj_gin_enc_study}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{lllllllllllll}
% \toprule
% Encoding &                ND &                N1 &                N2 &                N3 &                N4 &                NA &                FD &                F1 &                F2 &                F3 &                F4 &                FA \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]
% AdjOp              &  $0.960_{0.010}$ &  $0.737_{0.016}$ &  $0.630_{0.019}$ &  $0.712_{0.020}$ &  $0.733_{0.020}$ &  $0.587_{0.019}$ &  $0.680_{0.025}$ &  $0.290_{0.037}$ &\bR$0.678_{0.067}$ &  $0.526_{0.043}$ &  $0.719_{0.037}$ &  $0.477_{0.051}$ \\\cmidrule(lr){1-1} \cmidrule(lr){2-7} \cmidrule(lr){8-13} \addlinespace[0.5ex]

% (+ Arch2Vec) &\bR$0.965_{0.010}$ &  $0.756_{0.031}$ &\bR$0.641_{0.020}$ &  $0.700_{0.048}$ &  $0.722_{0.011}$ &\bR$0.608_{0.033}$ &  $0.721_{0.050}$ &  $0.372_{0.033}$ &  $0.641_{0.062}$ &\bR$0.613_{0.048}$ &\bR$0.762_{0.049}$ &\bR$0.556_{0.021}$ \\
% (+ CATE)     &  $0.964_{0.010}$ &  $0.764_{0.030}$ &  $0.637_{0.018}$ &  $0.706_{0.020}$ &  $0.720_{0.013}$ &  $0.604_{0.026}$ &  $0.688_{0.032}$ &  $0.388_{0.036}$ &  $0.578_{0.062}$ &  $0.478_{0.139}$ &  $0.752_{0.025}$ &  $0.516_{0.053}$ \\
% (+ CAZ)      &  $0.962_{0.007}$ &  $0.739_{0.024}$ &  $0.634_{0.016}$ &  $0.692_{0.031}$ &  $0.726_{0.008}$ &  $0.576_{0.013}$ &\bR$0.799_{0.042}$ &\bR$0.479_{0.053}$ &  $0.445_{0.045}$ &  $0.416_{0.057}$ &  $0.723_{0.036}$ &  $0.463_{0.014}$ \\
% (+ ZCP)      &  $0.964_{0.007}$ &\bR$0.759_{0.030}$ &  $0.636_{0.022}$ &\bR$0.708_{0.029}$ &\bR$0.739_{0.018}$ &  $0.596_{0.021}$ &  $0.793_{0.048}$ &  $0.479_{0.045}$ &  $0.490_{0.038}$ &  $0.444_{0.039}$ &  $0.746_{0.035}$ &  $0.484_{0.015}$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}
% \begin{table*}[t!]
%     \centering
%   \caption{Over three device sets on two NAS spaces, there is a benefit in using supplementary encodings for representing neural networks. CAZ was used as the sampler and 20 samples are fetched for transfer to ensure effective training of baseline predictor.}\vspace{2mm}
%   \label{table:adj_gin_enc_study}
%     \resizebox{\linewidth}{!}{%
% \begin{tabular}{lllllll}
% \toprule
% Task &                N0 &                N1 &                N2 &                N3 &                N4 &                N5 \\
% Encoding         &                  &                  &                  &                  &                  &                  \\
% % \midrule
%   \cmidrule(lr){1-1} \cmidrule(lr){2-7} \addlinespace[0.5ex]
% GIN              &  $0.960_{0.010}$ &  $0.737_{0.016}$ &  $0.630_{0.019}$ &  $0.712_{0.020}$ &  $0.733_{0.020}$ &  $0.587_{0.019}$ \\
% GIN$_{Arch2Vec}$ &\bR$0.965_{0.010}$ &  $0.756_{0.031}$ &\bR$0.641_{0.020}$ &  $0.700_{0.048}$ &  $0.722_{0.011}$ &\bR$0.608_{0.033}$ \\
% GIN$_{CATE}$     &  $0.964_{0.010}$ &  $0.764_{0.030}$ &  $0.637_{0.018}$ &  $0.706_{0.020}$ &  $0.720_{0.013}$ &  $0.604_{0.026}$ \\
% GIN$_{CAZ}$      &  $0.962_{0.007}$ &  $0.739_{0.024}$ &  $0.634_{0.016}$ &  $0.692_{0.031}$ &  $0.726_{0.008}$ &  $0.576_{0.013}$ \\
% GIN$_{ZCP}$      &  $0.964_{0.007}$ &\bR$0.759_{0.030}$ &  $0.636_{0.022}$ &\bR$0.708_{0.029}$ &\bR$0.739_{0.018}$ &  $0.596_{0.021}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{lllllll}
% \toprule
% Task &                F0 &                F1 &                F2 &                F3 &                F4 &                F5 \\
% Encoding         &                  &                  &                  &                  &                  &                  \\
% % \midrule
%   \cmidrule(lr){1-1} \cmidrule(lr){2-7} \addlinespace[0.5ex]
% GIN              &  $0.680_{0.025}$ &  $0.290_{0.037}$ &\bR$0.678_{0.067}$ &  $0.526_{0.043}$ &  $0.719_{0.037}$ &  $0.477_{0.051}$ \\
% GIN$_{Arch2Vec}$ &  $0.721_{0.050}$ &  $0.372_{0.033}$ &  $0.641_{0.062}$ &\bR$0.613_{0.048}$ &\bR$0.762_{0.049}$ &\bR$0.556_{0.021}$ \\
% GIN$_{CATE}$     &  $0.688_{0.032}$ &  $0.388_{0.036}$ &  $0.578_{0.062}$ &  $0.478_{0.139}$ &  $0.752_{0.025}$ &  $0.516_{0.053}$ \\
% GIN$_{CAZ}$      &\bR$0.799_{0.042}$ &\bR$0.479_{0.053}$ &  $0.445_{0.045}$ &  $0.416_{0.057}$ &  $0.723_{0.036}$ &  $0.463_{0.014}$ \\
% GIN$_{ZCP}$      &  $0.793_{0.048}$ &  $0.479_{0.045}$ &  $0.490_{0.038}$ &  $0.444_{0.039}$ &  $0.746_{0.035}$ &  $0.484_{0.015}$ \\
% \bottomrule
% \end{tabular}
%   }
%   \end{table*}

% \begin{table*}[t!]
%     \centering
%   \caption{Over three device sets on two NAS spaces, there is a benefit in using supplementary encodings for representing neural networks. CAZ was used as the sampler and 20 samples are fetched for transfer to ensure effective training of baseline predictor. \yash{running n0, n4, n5, f0, f4, f5 overnight}}\vspace{2mm}
%   \label{table:adj_gin_enc_study}
%     \resizebox{.8\linewidth}{!}{%
%   \begin{tabular}{lccccccc}
%   \toprule
%   Sampler &                N1 &                N2 &                N3&                F1 &                F2 &                F3 \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \addlinespace[0.5ex]
%     GIN              &  $0.759_{0.024}$ &  $0.663_{0.023}$ &  $0.744_{0.036}$ &  $0.693_{0.093}$ &\bB$0.790_{0.048}$ &  $0.623_{0.061}$ \\
%     GIN$_{Arch2Vec}$ &\bB$0.785_{0.030}$ &\bR$0.674_{0.026}$&\bB$0.747_{0.047}$ &\bR$0.770_{0.039}$&\bR$0.819_{0.048}$&\bR$0.706_{0.052}$\\
%     GIN$_{CATE}$     &\bR$0.789_{0.035}$&\bB$0.672_{0.021}$ &  $0.733_{0.020}$ &  $0.748_{0.043}$ &  $0.788_{0.047}$ &\bB$0.633_{0.110}$ \\
%     GIN$_{ZCP}$      &  $0.782_{0.030}$ &  $0.670_{0.031}$ &\bR$0.759_{0.021}$&\bB$0.757_{0.044}$ &  $0.749_{0.072}$ &  $0.570_{0.049}$ \\
%     GIN$_{CAZ}$      &  $0.773_{0.027}$ &  $0.671_{0.020}$ &  $0.722_{0.034}$ &  $0.739_{0.035}$ &  $0.757_{0.065}$ &  $0.525_{0.077}$ \\
%   \bottomrule
%   \end{tabular}
%   }
%   \end{table*}

% \begin{table*}[t!]
%     \centering
%   \caption{Over three device sets on two NAS spaces, there is a benefit in using supplementary encodings for representing neural networks. CAZ was used as the sampler and 20 samples are fetched for transfer to ensure effective training of baseline predictor. \yash{add n4 f4}}\vspace{2mm}
%   \label{table:adj_gin_enc_study}
%     \resizebox{.8\linewidth}{!}{%
% \begin{tabular}{llll}
% \toprule
% Task &                1 &                2 &                3 \\
% Encoding         &                  &                  &                  \\
% \midrule
% GIN              &  $0.737_{0.016}$ &  $0.630_{0.019}$ &  $0.712_{0.020}$ \\
% GIN$_{Arch2Vec}$ &  $0.756_{0.031}$ &  $0.641_{0.020}$ &  $0.700_{0.048}$ \\
% GIN$_{CATE}$     &  $0.764_{0.030}$ &  $0.637_{0.018}$ &  $0.706_{0.020}$ \\
% GIN$_{CAZ}$      &  $0.739_{0.024}$ &  $0.634_{0.016}$ &  $0.692_{0.031}$ \\
% GIN$_{ZCP}$      &  $0.759_{0.030}$ &  $0.636_{0.022}$ &  $0.708_{0.029}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{llll}
% \toprule
% Task &                1 &                2 &                3 \\
% Encoding         &                  &                  &                  \\
% \midrule
% GIN              &  $0.290_{0.037}$ &  $0.678_{0.067}$ &  $0.526_{0.043}$ \\
% GIN$_{Arch2Vec}$ &  $0.372_{0.033}$ &  $0.641_{0.062}$ &  $0.613_{0.048}$ \\
% GIN$_{CATE}$     &  $0.388_{0.036}$ &  $0.578_{0.062}$ &  $0.478_{0.139}$ \\
% GIN$_{CAZ}$      &  $0.479_{0.053}$ &  $0.445_{0.045}$ &  $0.416_{0.057}$ \\
% GIN$_{ZCP}$      &  $0.479_{0.045}$ &  $0.490_{0.038}$ &  $0.444_{0.039}$ \\
% \bottomrule
% \end{tabular}
%   }
%   \end{table*}

% \newpage 
% \newpage


% \begin{table}[h!]
%   \centering
% \caption{Using operation-wise hardware embedding to capture operation interactions as well as initializing hardware embeddings with the closest correlated device improve performance. 20 samples used for transfer. \yash{bar charts, geomeans, alternative presentations of data. SPLIT into two tables, one which shows effect of OpHW and other which shows HWInit}}\vspace{2mm}
% \label{table:hw_mlp_hwinit}
%   \resizebox{\linewidth}{!}{%
% \centering
% \begin{tabular}{cccc}
% \toprule
%  Device Set & Op$_{HW}$ & HWInit  &              SPR \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{ND}& \multirow{2}{*}{\ding{51}} & \ding{51} & \bR$0.806_{0.038}$ \\
%                     &   & \ding{55} &  $0.794_{0.038}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} &  $0.808_{0.027}$ \\
%                     &   & \ding{51} &  $0.804_{0.026}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N1} & \multirow{2}{*}{\ding{51}} & \ding{51} & \bR$0.719_{0.050}$ \\
%                     &   & \ding{55} &  $0.701_{0.046}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} &  $0.715_{0.041}$ \\
%                     &   & \ding{51} &  $0.701_{0.056}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N2} & \multirow{2}{*}{\ding{51}} & \ding{51} & \bR$0.795_{0.034}$ \\
%                     &   & \ding{55} &  $0.791_{0.036}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} &  $0.768_{0.036}$ \\
%                     &   & \ding{51} &  $0.763_{0.044}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N3}& \multirow{2}{*}{\ding{51}} & \ding{51} & $0.704_{0.058}$ \\
%                     &   & \ding{55} &  \bR$0.718_{0.055}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} &  $0.716_{0.039}$ \\
%                     &   & \ding{51} &  $0.680_{0.042}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N4}& \multirow{2}{*}{\ding{51}} & \ding{51} & $0.753_{0.052}$ \\
%                     &   & \ding{55} &  $0.750_{0.050}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} &  $0.717_{0.080}$ \\
%                     &   & \ding{51} &  \bR$0.757_{0.061}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{NA}& \multirow{2}{*}{\ding{51}} & \ding{51} & \bR$0.664_{0.059}$ \\
%                     &   & \ding{55} &  $0.658_{0.080}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} & $0.586_{0.066}$ \\
%                     &   & \ding{51} &  $0.660_{0.030}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{cccc}
%   \toprule
%    Device Set & Op$_{HW}$ & HWInit  &              SPR \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%   % \multirow{4}{*}{FD} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.770_{0.017}$ \\
%   %                     &   & \ding{55} &  $0.676_{0.092}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%   %                     & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.734_{0.050}$ \\
%   %                     &   & \ding{51} &  $0.766_{0.016}$ \\
%   \multirow{4}{*}{FD} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.845_{0.009}$ \\
%                       &   & \ding{55} &  $0.707_{0.158}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                       & \multirow{2}{*}{\ding{55}} &  \ding{55} & $0.791_{0.065}$ \\
%                       &   & \ding{51} &  $0.839_{0.010}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%   \multirow{4}{*}{F1} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.757_{0.048}$ \\
%                       &     & \ding{55} &  $0.609_{0.119}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                       & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.695_{0.067}$ \\
%                       &     & \ding{51} &  $0.753_{0.031}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%   \multirow{4}{*}{F2} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.769_{0.076}$ \\
%                       &   & \ding{55} &  $0.754_{0.064}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                       & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.715_{0.082}$ \\
%                       &   & \ding{51} &  $0.745_{0.081}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%   \multirow{4}{*}{F3} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.694_{0.076}$ \\
%                       &   & \ding{55} &  $0.655_{0.084}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                       & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.657_{0.078}$ \\
%                       &   & \ding{51} &  $0.685_{0.085}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%   \multirow{4}{*}{F4} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.832_{0.026}$ \\
%                       &   & \ding{55} &  $0.659_{0.158}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                       & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.785_{0.051}$ \\
%                       &   & \ding{51} &  $0.813_{0.030}$ \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%   \multirow{4}{*}{FA} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.628_{0.103}$ \\
%                       &   & \ding{55} &  $0.559_{0.118}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                       & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.579_{0.066}$ \\
%                       &   & \ding{51} &  $0.566_{0.081}$ \\
%   \bottomrule
%   \end{tabular}%
%   }
% \end{table}

% \begin{table}[t!]
%   \centering
% \caption{On NB201, GAT outperforms GCN significantly. On FBNet, the difference is less evident on FBNet. 20 samples used for transfer.\yash{TABLE DONE, Consider reformatting}}\vspace{2mm}
% \label{table:gcn_gat_design}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccc}
% \toprule
% Device Set & GNN Type &              SPR \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% % \midrule
% \multirow{3}{*}{ND}    &      GCN &  $0.814_{0.026}$ \\
%                        &      GAT &  $0.965_{0.005}$ \\
%                        &  GCN+GAT &  \bR$0.965_{0.011}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{N1}    &      GCN &  $0.741_{0.032}$ \\
%                        &      GAT &  \bR$0.848_{0.038}$ \\
%                        &  GCN+GAT &  $0.829_{0.046}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{N2}    &      GCN &  \bR$0.802_{0.021}$ \\
%                        &      GAT &  $0.612_{0.032}$ \\
%                        &  GCN+GAT &  $0.634_{0.029}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{N3}    &      GCN &  $0.710_{0.042}$ \\
%                        &      GAT &  $0.762_{0.039}$ \\
%                        &  GCN+GAT &  \bR$0.789_{0.054}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{ccc}
% \toprule
% Device Set & GNN Type &              SPR \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% % \midrule
% % \multirow{3}{*}{FD}    &      GCN &  $0.775_{0.006}$ \\
% %                        &      GAT &  $0.766_{0.013}$ \\
% %                        &  GCN+GAT &  \bR$0.798_{0.008}$ \\
% \multirow{3}{*}{FD}    &      GCN & \bR$0.844_{0.004}$  \\
%                        &      GAT &  $0.823_{0.019}$ \\
%                        &  GCN+GAT &  $0.835_{0.007}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{F1}    &      GCN &  $0.740_{0.055}$ \\
%                        &      GAT &  \bR$0.749_{0.042}$ \\
%                        &  GCN+GAT &  $0.733_{0.059}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{F2}    &      GCN &  $0.752_{0.076}$ \\
%                        &      GAT &  $0.700_{0.114}$ \\
%                        &  GCN+GAT &  \bR$0.766_{0.013}$  \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{F3}    &      GCN &  \bR$0.621_{0.120}$ \\
%                        &      GAT &  $0.589_{0.083}$ \\
%                        &  GCN+GAT &  $0.609_{0.106}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table*}[t!]
%   \centering
% \caption{exp631.py}\vspace{2mm}
% \label{table:exp631}
%   \resizebox{\linewidth}{!}{%
%   \begin{tabular}{llll}
% \toprule
% Task &                N1 &                N2 &                N3 \\
% Sampler    &                  &                  &                  \\
% \midrule
% a2vcatezcp &  $0.788_{0.088}$ &  $0.641_{0.024}$ &  $0.759_{0.041}$ \\
% arch2vec   &  $0.719_{0.068}$ &  $0.653_{0.028}$ &  $0.711_{0.062}$ \\
% cate       &  $0.799_{0.030}$ &  $0.649_{0.028}$ &  $0.824_{0.026}$ \\
% latency    &  $0.799_{0.094}$ &  $0.663_{0.026}$ &  $0.738_{0.097}$ \\
% params     &  $0.782_{0.090}$ &  $0.654_{0.033}$ &  $0.732_{0.081}$ \\
% random     &  $0.777_{0.087}$ &  $0.644_{0.038}$ &  $0.742_{0.069}$ \\
% zcp        &  $0.825_{0.022}$ &  $0.626_{0.027}$ &  $0.729_{0.078}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{llll}
% \toprule
% Task &                F1 &                F2 &                F3 \\
% Sampler    &                  &                  &                  \\
% \midrule
% a2vcatezcp &  $0.629_{0.138}$ &  $0.790_{0.040}$ &  $0.671_{0.055}$ \\
% arch2vec   &  $0.671_{0.067}$ &  $0.590_{0.088}$ &  $0.633_{0.072}$ \\
% cate       &  $0.145_{0.090}$ &  $0.489_{0.115}$ &  $0.276_{0.169}$ \\
% latency    &  $0.689_{0.130}$ &  $0.718_{0.080}$ &  $0.693_{0.050}$ \\
% params     &  $0.689_{0.130}$ &  $0.713_{0.087}$ &  $0.659_{0.095}$ \\
% random     &  $0.715_{0.095}$ &  $0.702_{0.075}$ &  $0.665_{0.085}$ \\
% zcp        &  $0.694_{0.040}$ &  $0.570_{0.127}$ &  $0.625_{0.050}$ \\
% \bottomrule
% \end{tabular}

%   }%
%   \end{table*}

% \begin{table*}[t!]
%   \centering
% \caption{exp632.py}\vspace{2mm}
% \label{table:exp632}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{llll}
% \toprule
% Task &                N1 &                N2 &                N3 \\
% Encoding         &                  &                  &                  \\
% \midrule
% GIN              &  $0.737_{0.016}$ &  $0.630_{0.019}$ &  $0.712_{0.020}$ \\
% GIN$_{Arch2Vec}$ &  $0.756_{0.031}$ &  $0.641_{0.020}$ &  $0.700_{0.048}$ \\
% GIN$_{CATE}$     &  $0.764_{0.030}$ &  $0.637_{0.018}$ &  $0.706_{0.020}$ \\
% GIN$_{CAZ}$      &  $0.739_{0.024}$ &  $0.634_{0.016}$ &  $0.692_{0.031}$ \\
% GIN$_{ZCP}$      &  $0.759_{0.030}$ &  $0.636_{0.022}$ &  $0.708_{0.029}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{llll}
% \toprule
% Task &                F1 &                F2 &                F3 \\
% Encoding         &                  &                  &                  \\
% \midrule
% GIN              &  $0.290_{0.037}$ &  $0.678_{0.067}$ &  $0.526_{0.043}$ \\
% GIN$_{Arch2Vec}$ &  $0.372_{0.033}$ &  $0.641_{0.062}$ &  $0.613_{0.048}$ \\
% GIN$_{CATE}$     &  $0.388_{0.036}$ &  $0.578_{0.062}$ &  $0.478_{0.139}$ \\
% GIN$_{CAZ}$      &  $0.479_{0.053}$ &  $0.445_{0.045}$ &  $0.416_{0.057}$ \\
% GIN$_{ZCP}$      &  $0.479_{0.045}$ &  $0.490_{0.038}$ &  $0.444_{0.039}$ \\
% \bottomrule
% \end{tabular}
%   }%
%   \end{table*}

% \begin{table*}[t!]
%   \centering
% \caption{exp622.py}\vspace{2mm}
% \label{table:exp622}
%   \resizebox{.7\linewidth}{!}{%
% \begin{tabular}{lll}
% \toprule
% {} & GNN Type &              SPR \\
% Task &          &                  \\
% \midrule
% 0    &  GCN+GAT &  $0.965_{0.011}$ \\
% 0    &      GCN &  $0.814_{0.026}$ \\
% 0    &      GAT &  $0.965_{0.005}$ \\
% 1    &      GAT &  $0.848_{0.038}$ \\
% 1    &      GCN &  $0.741_{0.032}$ \\
% 1    &  GCN+GAT &  $0.829_{0.046}$ \\
% 2    &      GAT &  $0.612_{0.032}$ \\
% 2    &  GCN+GAT &  $0.634_{0.029}$ \\
% 2    &      GCN &  $0.802_{0.021}$ \\
% 3    &      GCN &  $0.710_{0.042}$ \\
% 3    &  GCN+GAT &  $0.789_{0.054}$ \\
% 3    &      GAT &  $0.762_{0.039}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{lll}
% \toprule
% {} & GNN Type &              SPR \\
% Task &          &                  \\
% \midrule
% 0    &      GCN &  $0.775_{0.006}$ \\
% 0    &      GAT &  $0.766_{0.013}$ \\
% 0    &  GCN+GAT &  $0.768_{0.008}$ \\
% 1    &      GCN &  $0.740_{0.055}$ \\
% 1    &      GAT &  $0.749_{0.042}$ \\
% 1    &  GCN+GAT &  $0.733_{0.059}$ \\
% 2    &      GCN &  $0.752_{0.076}$ \\
% 2    &      GAT &  $0.700_{0.114}$ \\
% 2    &  GCN+GAT &  $0.740_{0.089}$ \\
% 3    &      GCN &  $0.621_{0.120}$ \\
% 3    &      GAT &  $0.589_{0.083}$ \\
% 3    &  GCN+GAT &  $0.609_{0.106}$ \\
% \bottomrule
% \end{tabular}
%   }%
%   \end{table*}


% \begin{table*}[t!]
%   \centering
% \caption{exp621.py}\vspace{2mm}
% \label{table:exp621}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{llll}
% \toprule
% {} & HWEmb$\longrightarrow$MLP & Transfer HWEmb &              SPR \\
% Task &                           &                &                  \\
% \midrule
% 0    &                 \ding{51} &      \ding{51} &  $0.834_{0.026}$ \\
% 0    &                 \ding{55} &      \ding{55} &  $0.794_{0.038}$ \\
% 0    &                 \ding{51} &      \ding{55} &  $0.808_{0.027}$ \\
% 0    &                 \ding{55} &      \ding{51} &  $0.806_{0.038}$ \\
% 1    &                 \ding{55} &      \ding{51} &  $0.719_{0.050}$ \\
% 1    &                 \ding{55} &      \ding{55} &  $0.701_{0.046}$ \\
% 1    &                 \ding{51} &      \ding{55} &  $0.715_{0.041}$ \\
% 1    &                 \ding{51} &      \ding{51} &  $0.701_{0.056}$ \\
% 2    &                 \ding{55} &      \ding{51} &  $0.795_{0.034}$ \\
% 2    &                 \ding{55} &      \ding{55} &  $0.791_{0.036}$ \\
% 2    &                 \ding{51} &      \ding{51} &  $0.763_{0.044}$ \\
% 2    &                 \ding{51} &      \ding{55} &  $0.768_{0.036}$ \\
% 3    &                 \ding{55} &      \ding{55} &  $0.718_{0.055}$ \\
% 3    &                 \ding{51} &      \ding{55} &  $0.716_{0.039}$ \\
% 3    &                 \ding{55} &      \ding{51} &  $0.704_{0.058}$ \\
% 3    &                 \ding{51} &      \ding{51} &  $0.680_{0.042}$ \\
% \bottomrule
% \end{tabular}


%   \begin{tabular}{llll}
% \toprule
% {} & HWEmb$\longrightarrow$MLP & Transfer HWEmb &              SPR \\
% Task &                           &                &                  \\
% \midrule
% 0    &                 \ding{55} &      \ding{51} &  $0.770_{0.017}$ \\
% 0    &                 \ding{55} &      \ding{55} &  $0.676_{0.092}$ \\
% 0    &                 \ding{51} &      \ding{55} &  $0.734_{0.050}$ \\
% 0    &                 \ding{51} &      \ding{51} &  $0.766_{0.016}$ \\
% 1    &                 \ding{55} &      \ding{51} &  $0.757_{0.048}$ \\
% 1    &                 \ding{51} &      \ding{51} &  $0.753_{0.031}$ \\
% 1    &                 \ding{51} &      \ding{55} &  $0.695_{0.067}$ \\
% 1    &                 \ding{55} &      \ding{55} &  $0.609_{0.119}$ \\
% 2    &                 \ding{51} &      \ding{51} &  $0.769_{0.076}$ \\
% 2    &                 \ding{55} &      \ding{55} &  $0.715_{0.082}$ \\
% 2    &                 \ding{51} &      \ding{55} &  $0.745_{0.081}$ \\
% 2    &                 \ding{55} &      \ding{51} &  $0.754_{0.064}$ \\
% 3    &                 \ding{55} &      \ding{51} &  $0.655_{0.084}$ \\
% 3    &                 \ding{51} &      \ding{51} &  $0.694_{0.076}$ \\
% 3    &                 \ding{51} &      \ding{55} &  $0.685_{0.085}$ \\
% 3    &                 \ding{55} &      \ding{55} &  $0.657_{0.078}$ \\
% \bottomrule
% \end{tabular}
%   }%
%   \end{table*}


% \begin{table*}[t!]
%   \centering
% \caption{exp621.py}\vspace{2mm}
% \label{table:exp621}
%   \resizebox{\linewidth}{!}{%
%   \begin{tabular}{ccccc}
% \toprule
%   & N0 & N1 & N2 & N5 \\
% \hline
% GIN & $0.994_{0.002}$ & $0.951_{0.006}$ & $0.844_{0.037}$ & $0.992_{0.003}$ \\
% (+TransferEmb) & $0.992_{0.002}$ & $0.953_{0.004}$ & $0.865_{0.026}$ & $0.990_{0.007}$ \\
% (+Op-HWEmb) & $0.992_{0.003}$ & $0.957_{0.007}$ & $0.884_{0.020}$ & $0.994_{0.004}$ \\
% (+Sampler) & $0.991_{0.003}$ & $0.949_{0.010}$ & $0.830_{0.040}$ & $0.991_{0.002}$ \\
% (+Supplementary Encoding) & $0.992_{0.003}$ & $0.943_{0.008}$ & $0.836_{0.025}$ & $0.992_{0.002}$ \\
% \end{tabular}


%   \begin{tabular}{ccccc}
% \toprule
%   & F0 & F1 & F2 & F4 \\
% \hline
% GIN & $0.840_{0.065}$ & $0.772_{0.071}$ & $0.713_{0.094}$ & $0.875_{0.023}$ \\
% (+TransferEmb) & $0.930_{0.008}$ & $0.805_{0.046}$ & $0.830_{0.022}$ & $0.887_{0.021}$ \\
% (+Op-HWEmb) & $0.933_{0.012}$ & $0.842_{0.028}$ & $0.842_{0.012}$ & $0.906_{0.008}$ \\
% (+Sampler) & $0.937_{0.005}$ & $0.844_{0.020}$ & $0.840_{0.008}$ & $0.909_{0.005}$ \\
% (+Supplementary Encoding) & - & $0.905_{0.011}$ & $0.841_{0.011}$ & $0.942_{0.007}$ \\
% \end{tabular}
%   }%
%   \end{table*}

  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\end{document}


% This document was modified from the file originally made available by
% Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% by Iain Murray in 2018. It was modified from a version from Dan Roy in
% 2017, which was based on a version from Lise Getoor and Tobias
% Scheffer, which was slightly modified from the 2010 version by
% Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% slightly modified from Prasad Tadepalli's 2007 version which is a
% lightly changed version of the previous year's version by Andrew
% Moore, which was in turn edited from those of Kristian Kersting and
% Codrina Lauth. Alex Smola contributed to the algorithmic style files.


% \begin{table*}[t!]
%   \centering
% \caption{On the default (D) and adversarial (A) tasks introduced in HELP and MultiPredict, our predictor with the CAZ and CATE sampler works best for NASBench-201 and FBNet respectively. Standard deviations are reported for results we report.}\vspace{2mm}
% \label{table:all_final_results}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccccccccccccccccc}
% \toprule
%   & Source & Target             & \multirow{2}{*}{ND} & \multirow{2}{*}{NA} & \multirow{2}{*}{N1} & \multirow{2}{*}{N2} & \multirow{2}{*}{N3} & \multirow{2}{*}{N4} & Source & Target             & \multirow{2}{*}{FD} & \multirow{2}{*}{FA} & \multirow{2}{*}{F1} & \multirow{2}{*}{F2} & \multirow{2}{*}{F3} & \multirow{2}{*}{F4} \\
%   & \multicolumn{2}{c}{Samples} &  &  &  &  & & & \multicolumn{2}{c}{Samples} &  &  &  &  & &\\
  
%   % \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-13} \addlinespace[0.5ex]
%   \midrule
% % MultiPredict        & 900 &  10  & 0.94               & 0.78 & $0.949_{0.024}$  & $0.746_{0.102}$  & $0.947_{0.15}$ & $0.956_{0.004}$ & 4000 & 10 &  \\
% % HELP                & 900 &  20  & 0.93               & 0.36 & $0.949_{0.0204}$ & $0.694_{0.045}$  & $0.944_{0.018}$ & $0.939_{0.024}$ & 4000 & 20 &  \\
% % MultiPredict        & 900 &  10   & 4000 & 10 &  \\
% % HELP                & 900 &  20 & $0.816_{0.110}$ & $0.405_{0.043}$ & $0.865_{0.162}$ & $0.744_{0.167}$ & $0.837_{0.110}$ & $0.712_{0.062}$ &  4000 & 20 & $0.596_{0.286}$ & $0.406_{0.007}$ & $0.793_{0.028}$ & $0.543_{0.036}$ & $0.586_{0.239}$ & $0.610_{0.164}$   \\
% HELP                & 900 &  20 & $0.948_{0.006}$ & $0.410_{0.037}$ & $0.604_{0.044}$ & $0.509_{0.007}$ & $0.729_{0.027}$ & $0.746_{0.042}$ &  4000 & 20 & $0.965_{0.001}$ & $0.406_{0.007}$ & $0.793_{0.028}$ & $0.543_{0.036}$ & $0.413_{0.015}$ & $0.799_{0.004}$   \\
% MultiPredict        & 900 &  20 & $0.930_{0.012}$ & $0.820_{0.019}$ & $0.970_{0.003}$ & $0.757_{0.045}$ & $0.947_{0.012}$ & $0.952_{0.011}$ &  4000 & 20 & $0.944_{0.012}$ & $0.000_{0}$ & $0.756_{0.026}$ & $0.567_{0.075}$ & $0.434_{0.040}$ & $0.763_{0.011}$    \\
%             Ours    & 25 &  20  & \bR$0.959_{0.007}$ & \bR$0.893_{0.036}$ & \bR$0.967_{0.007}$ & \bR$0.857_{0.029}$ & \bR$0.962_{0.008}$ & \bR$0.959_{0.012}$ & 200  & 20 &  $0.729_{0.070}$ & $0.507_{0.122}$  & $0.704_{0.059}$ & $0.829_{0.034}$ & $0.831_{0.054}$ & $0.698_{0.091}$\\
%             % Ours    & 25 &  20  & \bR$0.959_{0.007}$ & \bR$0.893_{0.036}$ & \bR$0.967_{0.007}$ & \bR$0.857_{0.029}$ & \bR$0.962_{0.008}$ & \bR$0.959_{0.012}$ & 200  & 20 & $0.923_{0.010}$ &  \bR$0.682_{0.112}$  & $0.802_{0.012}$ & $0.808_{0.056}$ & $0.809_{0.064}$ & $0.868_{0.024}$ \\
%             % Ours    & 900 &  20  & $0.992_{0.003}$    & $0.994_{0.004}$         & \bR$0.957_{0.007}$ & \bR$0.884_{0.020}$ & & & 4000 & 20 & $0.937_{0.005}$ &    &  \bR$0.905_{0.011}$ & & & \bR$0.942_{0.007}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


% \begin{table}[h!]
%   \centering
% \caption{Using operation-wise hardware embedding to capture operation interactions as well as initializing hardware embeddings with the closest correlated device improve performance. 20 samples used for transfer.}\vspace{2mm}
% \label{table:hw_mlp_hwinit}
%   \resizebox{\linewidth}{!}{%
% \centering
% \begin{tabular}{cccc}
% \toprule
%  Device Set & Op$_{HW}$ & HWInit  &              SPR \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N1} & \multirow{2}{*}{\ding{51}} & \ding{51} & \bR$0.719_{0.050}$ \\
%                     &   & \ding{55} &  $0.701_{0.046}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} &  $0.715_{0.041}$ \\
%                     &   & \ding{51} &  $0.701_{0.056}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N2} & \multirow{2}{*}{\ding{51}} & \ding{51} & \bR$0.795_{0.034}$ \\
%                     &   & \ding{55} &  $0.791_{0.036}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} & \ding{55} &  $0.768_{0.036}$ \\
%                     &   & \ding{51} &  $0.763_{0.044}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{cccc}
% \toprule
%  Device Set & Op$_{HW}$ & HWInit  &              SPR \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{F0} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.770_{0.017}$ \\
%                     &   & \ding{55} &  $0.676_{0.092}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.734_{0.050}$ \\
%                     &   & \ding{51} &  $0.766_{0.016}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{F1} & \multirow{2}{*}{\ding{51}} &  \ding{51} & \bR$0.757_{0.048}$ \\
%                     &     & \ding{55} &  $0.609_{0.119}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{55}} &  \ding{55} &  $0.695_{0.067}$ \\
%                     &     & \ding{51} &  $0.753_{0.031}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
% \begin{figure*}
%     \centering
%     \caption{Standard deviation of neural network samplers using supplementary encodings are generally lower than random methods.}
%     \label{fig:sampler_stdev}
%     \includegraphics[width=\linewidth]{mlsys2024style/figures/sampler_stddev.pdf}
%     % \vspace{-3mm}
% \end{figure*}



% \begin{table}[t!]
%   \centering
% \caption{On NB201, GAT outperforms GCN significantly. On FBNet, the difference is less evident on FBNet. 20 samples used for transfer.}\vspace{2mm}
% \label{table:gcn_gat_design}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccc}
% \toprule
% Device Set & GNN Type &              SPR \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% % \midrule
% \multirow{3}{*}{N0}    &      GCN &  $0.814_{0.026}$ \\
%                        &      GAT &  $0.965_{0.005}$ \\
%                        &  GCN+GAT &  \bR$0.965_{0.011}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{N3}    &      GCN &  $0.710_{0.042}$ \\
%                        &      GAT &  $0.762_{0.039}$ \\
%                        &  GCN+GAT &  \bR$0.789_{0.054}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{ccc}
% \toprule
% Device Set & GNN Type &              SPR \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% % \midrule
% \multirow{3}{*}{F0}    &      GCN &  $0.775_{0.006}$ \\
%                        &      GAT &  $0.766_{0.013}$ \\
%                        &  GCN+GAT &  \bR$0.798_{0.008}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \multirow{3}{*}{F3}    &      GCN &  \bR$0.621_{0.120}$ \\
%                        &      GAT &  $0.589_{0.083}$ \\
%                        &  GCN+GAT &  $0.609_{0.106}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[t!]
%   \centering
% \caption{We study the impact of design choices on the performacne of predictors on three FBNet device sets.}\vspace{2mm}
% \label{table:design_components}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{lccc}
% \toprule
%                               & F1 & F2 & F4 \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-4} \addlinespace[0.5ex]
% GIN                            & $0.772_{0.071}$ & $0.713_{0.094}$ & $0.875_{0.023}$ \\
% (+ HWInit)                     & $0.805_{0.046}$ & $0.830_{0.022}$ & $0.887_{0.021}$ \\
% (+ Op$_{HW}$)                  & \bB$0.842_{0.028}$ & \bR$0.842_{0.012}$ & $0.906_{0.008}$ \\
% (+ Sampler)                    & $0.844_{0.020}$ & $0.840_{0.008}$ & \bB$0.909_{0.005}$ \\
% (+ Supp. Encoding)             & \bR$0.905_{0.011}$ & \bB$0.841_{0.011}$ & \bR$0.942_{0.007}$ \\
% \bottomrule

% \end{tabular}%
% }
% \end{table}




% \begin{table*}[t!]
%   \centering
% \caption{On the default (D) and adversarial (A) tasks introduced in HELP and MultiPredict, our predictor with the CAZ and CATE sampler works best for NASBench-201 and FBNet respectively. Standard deviations are reported for results we report.}\vspace{2mm}
% \label{table:all_final_results}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccccccccccccccccc}
% \toprule
%   & Source & Target             & \multirow{2}{*}{ND} & \multirow{2}{*}{NA} & \multirow{2}{*}{N1} & \multirow{2}{*}{N2} & \multirow{2}{*}{N3} & \multirow{2}{*}{N4} & Source & Target             & \multirow{2}{*}{FD} & \multirow{2}{*}{FA} & \multirow{2}{*}{F1} & \multirow{2}{*}{F2} & \multirow{2}{*}{F3} & \multirow{2}{*}{F4} \\
%   & \multicolumn{2}{c}{Samples} &  &  &  &  & & & \multicolumn{2}{c}{Samples} &  &  &  &  & &\\
  
%   % \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-13} \addlinespace[0.5ex]
%   \midrule
% MultiPredict        & 900 &  10  & 0.94               & 0.78 & $0.949_{0.024}$  & $0.746_{0.102}$  &  &  & 4000 & 10 & \bR$0.96$           & 0.45            & $0.770_{0.054}$ & &  & $0.764_{0.087}$  \\
% HELP                & 900 &  20  & 0.93               & 0.36 & $0.949_{0.0204}$ & $0.694_{0.045}$  & $0.944_{0.018}$ & $0.939_{0.024}$ & 4000 & 20 & 0.91                & 0.37            & $0.909_{0.000}$  & & & $0.826_{0.001}$  \\
%             Ours    & 25 &  20  & \bR$0.993_{0.003}$ &  \bR$0.994_{0.001}$     & $0.950_{0.007}$    & $0.866_{0.011}$& \bR$0.954_{0.003}$ & \bR$0.955_{0.004}$  & 200  & 20 & $0.923_{0.010}$ &  \bR$0.682_{0.112}$  & $0.802_{0.012}$ & $0.808_{0.056}$ & $0.809_{0.064}$ & $0.868_{0.024}$ \\
%             Ours    & 900 &  20  & $0.992_{0.003}$    & $0.994_{0.004}$         & \bR$0.957_{0.007}$ & \bR$0.884_{0.020}$ & & & 4000 & 20 & $0.937_{0.005}$ &    &  \bR$0.905_{0.011}$ & & & \bR$0.942_{0.007}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}
% \begin{table*}[t!]
%   \centering
% \caption{On the default (D) and adversarial (A) tasks introduced in HELP and MultiPredict, our predictor with the CAZ and CATE sampler works best for NASBench-201 and FBNet respectively. Standard deviations are reported for results we report.}\vspace{2mm}
% \label{table:all_final_results}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccccccccccccc}
% \toprule
%   & Source & Target             & \multirow{2}{*}{ND} & \multirow{2}{*}{NA} & \multirow{2}{*}{N1} & \multirow{2}{*}{N2} & Source & Target             & \multirow{2}{*}{FD} & \multirow{2}{*}{FA} & \multirow{2}{*}{F1} & \multirow{2}{*}{F4} \\
%   & \multicolumn{2}{c}{Samples} &  &  &  &  & \multicolumn{2}{c}{Samples} &  &  &  &  \\
  
%   \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-13} \addlinespace[0.5ex]
% MultiPredict        & 900 &  10  & 0.94               & 0.78 & $0.949_{0.024}$  & $0.746_{0.102}$    & 4000 & 10 & \bR$0.96$           & 0.45            & $0.770_{0.054}$ & $0.764_{0.087}$  \\
% HELP                & 900 &  20  & 0.93               & 0.36 & $0.949_{0.0204}$ & $0.694_{0.045}$    & 4000 & 20 & 0.91                & 0.37            & $0.909_{0.000}$ & $0.826_{0.001}$  \\
%             Ours    & 25 &  20  & \bR$0.993_{0.003}$ &  \bR$0.994_{0.001}$     & $0.950_{0.007}$    & $0.866_{0.011}$    & 200  & 20 & $0.923_{0.010}$ &  \bR$0.682_{0.112}$  & $0.802_{0.012}$ & $0.868_{0.024}$ \\
%             Ours    & 900 &  20  & $0.992_{0.003}$    & $0.994_{0.004}$         & \bR$0.957_{0.007}$ & \bR$0.884_{0.020}$ & 4000 & 20 & $0.937_{0.005}$ &    &  \bR$0.905_{0.011}$ & \bR$0.942_{0.007}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

% \begin{table}[t!]
%   \centering
% \caption{We study the impact of design choices on the performacne of predictors on three FBNet device sets.}\vspace{2mm}
% \label{table:design_components}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
%   & F0 & F1 & F2 & F3 & F4 & F5 \\
%   \cmidrule(lr){1-1} \cmidrule(lr){2-7} \addlinespace[0.5ex]
% GIN                & $0.923_{0.010}$ & $0.827_{0.020}$ & $0.801_{0.109}$ & $0.776_{0.069}$ & $0.860_{0.020}$ & $0.495_{0.126}$ \\
% (+HWInit)          & $0.922_{0.014}$ & $0.805_{0.027}$ & $0.804_{0.079}$ & $0.761_{0.083}$ & $0.866_{0.034}$ & $0.582_{0.069}$ \\
% (+Op$_{HW}$)       & $0.905_{0.029}$ & $0.755_{0.055}$ & $0.831_{0.051}$ & $0.672_{0.214}$ & $0.868_{0.024}$ & $0.682_{0.112}$ \\
% (+Sampler)         & $0.903_{0.016}$ & $0.802_{0.012}$ & $0.873_{0.010}$ & $0.666_{0.200}$ & $0.858_{0.038}$ & $0.529_{0.074}$ \\
% (+Supp. Encoding)  & $0.922_{0.016}$ & $0.819_{0.042}$ & $0.808_{0.056}$ & $0.809_{0.064}$ & $0.859_{0.038}$ & $0.466_{0.059}$ \\

% \bottomrule

% \end{tabular}%
% }
% \end{table}

% \begin{table}[t!]
%   \centering
% \caption{On NB201, 25 pre-training samples (vs 900 for HELP), 20 samples from target device.}\vspace{2mm}
% \label{table:nb201_final_results}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccccccc}
%   & N0 & N1 & N2 & N3 & N4 & N5 \\
% \hline
% HELP & $0.931_{0.013}$ & $0.949_{0.020}$ & $0.694_{0.045}$ & $0.944_{0.018}$ & $0.938_{0.024}$ & $0.93$ \\\midrulex
% GIN & $0.993_{0.003}$ & $0.949_{0.014}$ & $0.860_{0.012}$ & $0.952_{0.012}$ & $0.958_{0.005}$ & $0.991_{0.005}$ \\
% (+TransferEmb) & $0.993_{0.003}$ & $0.950_{0.007}$ & $0.872_{0.018}$ & $0.950_{0.013}$ & $0.960_{0.005}$ & $0.992_{0.005}$ \\
% (+Op-HWEmb) & $0.992_{0.004}$ & $0.950_{0.007}$ & $0.866_{0.011}$ & $0.954_{0.003}$ & $0.955_{0.004}$ & $0.994_{0.001}$ \\
% (+Sampler) & $0.991_{0.002}$ & $0.945_{0.011}$ & $0.856_{0.008}$ & $0.939_{0.018}$ & $0.948_{0.007}$ & $0.991_{0.004}$ \\
% (+Supplementary Encoding) & $0.984_{0.007}$ & $0.947_{0.008}$ & $0.850_{0.007}$ & $0.941_{0.015}$ & $0.947_{0.011}$ & - \\
% % GIN & $0.993_{0.003}$ & $0.949_{0.014}$ & $0.860_{0.012}$ & $0.952_{0.012}$ & $0.958_{0.005}$ \\
% % (+TransferEmb) & $0.993_{0.003}$ & $0.950_{0.007}$ & $0.872_{0.018}$ & $0.950_{0.013}$ & $0.960_{0.005}$ \\
% % Our Best & $0.992_{0.004}$ & $0.950_{0.007}$ & $0.866_{0.011}$ & $0.954_{0.003}$ & $0.955_{0.004}$ \\
% % (+Sampler) & $0.991_{0.002}$ & $0.945_{0.011}$ & $0.856_{0.008}$ & $0.939_{0.018}$ & $0.948_{0.007}$ \\
% % (+Supplementary Encoding) & $0.984_{0.007}$ & $0.947_{0.008}$ & $0.850_{0.007}$ & $0.941_{0.015}$ & $0.947_{0.011}$ \\
% \end{tabular}%
% }
% \end{table}

% \begin{table}[t!]
%   \centering
% \caption{On FBNet, 200 pre-training samples (vs 4000 for HELP), 20 samples from target device.}\vspace{2mm}
% \label{table:fbnet_final_results}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{cccccc}
%   & F0 & F1 & F2 & F3 & F4 \\
% \hline
% HELP & & & & &  \\\midrule
% GIN & $0.000_{0.000}$ & $0.000_{0.000}$ & $0.000_{0.000}$ & $0.000_{0.000}$ & $0.712_{0.288}$ \\
% (+TransferEmb) & $0.918_{0.034}$ & $0.806_{0.025}$ & $0.715_{0.304}$ & $0.843_{0.056}$ & $0.857_{0.040}$ \\
% (+Op-HWEmb) & $0.000_{0.000}$ & $0.807_{0.040}$ & $0.000_{0.000}$ & $0.000_{0.000}$ & $0.000_{0.000}$ \\
% (+Sampler) & $0.911_{0.029}$ & $0.000_{0.000}$ & $0.772_{0.108}$ & $0.000_{0.000}$ & $0.633_{0.400}$ \\
% (+Supplementary Encoding) & $0.958_{0.013}$ & $0.733_{0.085}$ & $0.856_{0.090}$ & $0.869_{0.044}$ & $0.897_{0.033}$ \\
% \end{tabular}%
% }
% \end{table}

% \begin{table}[t!]
%   \centering
% \caption{On NB201, supplementary encodings enable better samplers. The difference is less evident on FBNet.}\vspace{2mm}
% \label{table:sampler_study}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% Sampler &                N1 &                N2 &                N3&                F1 &                F2 &                F3 \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \addlinespace[0.5ex]
% Random              &  $0.784_{0.076}$ &  $0.635_{0.034}$ &  $0.712_{0.073}$ &  $0.686_{0.112}$ &  $0.669_{0.049}$ &  $0.603_{0.061}$ \\
% Latency (Oracle)    &  $0.810_{0.060}$ &  $0.648_{0.014}$ &  $0.737_{0.103}$ &  $0.649_{0.140}$ &  \bB$0.681_{0.035}$ &  \bB$0.640_{0.085}$ \\
% Params              &  \bB$0.817_{0.044}$ &  \bB$0.649_{0.024}$ &  \bB$0.777_{0.050}$ &  \bR$0.726_{0.049}$ &  \bR$0.739_{0.054}$ &  \bR$0.677_{0.033}$ \\
% Arch2Vec            &  $0.740_{0.053}$ &  \bR$0.654_{0.021}$ &  $0.728_{0.060}$ &  $0.658_{0.079}$ &  $0.616_{0.089}$ &  $0.574_{0.037}$ \\
% CATE                &  $0.814_{0.027}$ &  $0.634_{0.018}$ &  \bR$0.834_{0.019}$ &  $0.133_{0.032}$ &  $0.451_{0.152}$ &  $0.229_{0.135}$ \\
% ZCP                 &  \bR$0.822_{0.019}$ &  $0.623_{0.020}$ &  $0.722_{0.084}$ &  \bB$0.686_{0.024}$ &  $0.553_{0.136}$ &  $0.594_{0.067}$ \\
% CAZ                 &  $0.790_{0.069}$ &  $0.629_{0.016}$ &  $0.743_{0.044}$    &  - & - & -  \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{tabular}{llll}
% \toprule
% Task &                1 &                2 &                3 \\
% Sampler  &                  &                  &                  \\
% \midrule
% arch2vec &  $0.766_{0.017}$ &  $0.798_{0.030}$ &  $0.638_{0.056}$ \\
% cate     &  $0.109_{0.042}$ &  $0.465_{0.212}$ &  $0.278_{0.152}$ \\
% latency  &  $0.776_{0.015}$ &  $0.828_{0.016}$ &  $0.726_{0.104}$ \\
% params   &  $0.742_{0.058}$ &  $0.819_{0.037}$ &  $0.751_{0.028}$ \\
% random   &  $0.744_{0.054}$ &  $0.828_{0.019}$ &  $0.718_{0.060}$ \\
% zcp      &  $0.717_{0.043}$ &  $0.744_{0.062}$ &  $0.708_{0.040}$ \\
% \bottomrule
% \end{tabular}%

% \begin{table}[t!]
%   \centering
% \caption{On NB201, GAT outperforms GCN significantly. On FBNet, the difference is less evident on FBNet.}\vspace{2mm}
% \label{table:gcn_gat_design}
%   \resizebox{\linewidth}{!}{%
% \begin{tabular}{llll}
% \toprule
% Task &                1 &                2 &                3 \\
% Sampler    &                  &                  &                  \\
% \midrule
% % a2vcatezcp &  $0.860_{0.021}$ &  $0.696_{0.018}$ &  $0.810_{0.023}$ \\
% % accuracy   &  $0.886_{0.025}$ &  $0.715_{0.037}$ &  $0.874_{0.023}$ \\
% arch2vec   &  $0.879_{0.022}$ &  $0.726_{0.021}$ &  $0.859_{0.035}$ \\
% cate       &  $0.858_{0.026}$ &  $0.683_{0.022}$ &  $0.863_{0.050}$ \\
% latency    &  $0.884_{0.026}$ &  $0.717_{0.021}$ &  $0.855_{0.033}$ \\
% params     &  $0.869_{0.013}$ &  $0.715_{0.037}$ &  $0.874_{0.023}$ \\
% random     &  $0.886_{0.032}$ &  $0.693_{0.033}$ &  $0.808_{0.048}$ \\
% zcp        &  $0.838_{0.024}$ &  $0.681_{0.024}$ &  $0.857_{0.018}$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{llll}
% \toprule
% Task &                1 &                2 &                3 \\
% Sampler  &                  &                  &                  \\
% \midrule
% arch2vec &  $0.766_{0.017}$ &  $0.798_{0.030}$ &  $0.638_{0.056}$ \\
% cate     &  $0.109_{0.042}$ &  $0.465_{0.212}$ &  $0.278_{0.152}$ \\
% latency  &  $0.776_{0.015}$ &  $0.828_{0.016}$ &  $0.726_{0.104}$ \\
% params   &  $0.742_{0.058}$ &  $0.819_{0.037}$ &  $0.751_{0.028}$ \\
% random   &  $0.744_{0.054}$ &  $0.828_{0.019}$ &  $0.718_{0.060}$ \\
% zcp      &  $0.717_{0.043}$ &  $0.744_{0.062}$ &  $0.708_{0.040}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% 1    &      GCN &  $0.741_{0.032}$ \\
% 1    &      GAT &  $0.848_{0.038}$ \\
% 1    &  GCN+GAT &  $0.829_{0.046}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% 2    &      GCN &  $0.802_{0.021}$ \\
% 2    &      GAT &  $0.612_{0.032}$ \\
% 2    &  GCN+GAT &  $0.634_{0.029}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% 1    &      GCN &  $0.740_{0.055}$ \\
% 1    &      GAT &  $0.749_{0.042}$ \\
% 1    &  GCN+GAT &  $0.733_{0.059}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% 2    &      GCN &  $0.752_{0.076}$ \\
% 2    &      GAT &  $0.700_{0.114}$ \\
% 2    &  GCN+GAT &  $0.740_{0.089}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \addlinespace[0.5ex]
% \begin{table}[t!]
%   \centering
%   \resizebox{.6\linewidth}{!}{%
% \centering
% \begin{tabular}{cccc}
% \toprule
%  Device Set & HW$_{MLP}$ & HWInit  &              SPR \\
% % Task &                           &                &                  \\
% % \midrule
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N1} & \multirow{2}{*}{\ding{55}} & \ding{51} & \bR$0.719_{0.050}$ \\
%                     &   & \ding{55} &  $0.701_{0.046}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{51}} & \ding{55} &  $0.715_{0.041}$ \\
%                     &   & \ding{51} &  $0.701_{0.056}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N2} & \multirow{2}{*}{\ding{55}} & \ding{51} & \bR$0.795_{0.034}$ \\
%                     &   & \ding{55} &  $0.791_{0.036}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{51}} & \ding{55} &  $0.768_{0.036}$ \\
%                     &   & \ding{51} &  $0.763_{0.044}$ \\
% % \midrule
% %  & HWEmb$\longrightarrow$MLP & Transfer HWEmb &              SPR \\
% % Task &                           &                &                  \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{F0} & \multirow{2}{*}{\ding{55}} &  \ding{51} & \bR$0.770_{0.017}$ \\
%                     &   & \ding{55} &  $0.676_{0.092}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{51}} &  \ding{55} &  $0.734_{0.050}$ \\
%                     &   & \ding{51} &  $0.766_{0.016}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{F1} & \multirow{2}{*}{\ding{55}} &  \ding{51} & \bR$0.757_{0.048}$ \\
%                     &     & \ding{55} &  $0.609_{0.119}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \multirow{2}{*}{\ding{51}} &  \ding{55} &  $0.695_{0.067}$ \\
%                     &     & \ding{51} &  $0.753_{0.031}$ \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Using operation-wise hardware embedding to capture operation interactions as well as initializing hardware embeddings with the closest correlated device improve performance.}
% \label{table:hw_mlp_hwinit}
% \end{table}

% \begin{table}[t!]
%   \centering
%   \resizebox{.6\linewidth}{!}{%
% \centering
% \begin{tabular}{cccc}
% \toprule
%  Device Set & HW$_{MLP}$ & HWInit  &              SPR \\
% % Task &                           &                &                  \\
% % \midrule
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N1} & \ding{55} & \ding{51} & \bR$0.719_{0.050}$ \\
%                     & \ding{55} & \ding{55} &  $0.701_{0.046}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \ding{51} & \ding{55} &  $0.715_{0.041}$ \\
%                     & \ding{51} & \ding{51} &  $0.701_{0.056}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{N2} & \ding{55} & \ding{51} & \bR$0.795_{0.034}$ \\
%                     & \ding{55} & \ding{55} &  $0.791_{0.036}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \ding{51} & \ding{55} &  $0.768_{0.036}$ \\
%                     & \ding{51} & \ding{51} &  $0.763_{0.044}$ \\
% % \midrule
% %  & HWEmb$\longrightarrow$MLP & Transfer HWEmb &              SPR \\
% % Task &                           &                &                  \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{F0} & \ding{55} & \ding{51} & \bR$0.770_{0.017}$ \\
%                     & \ding{55} & \ding{55} &  $0.676_{0.092}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \ding{51} & \ding{55} &  $0.734_{0.050}$ \\
%                     & \ding{51} & \ding{51} &  $0.766_{0.016}$ \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
% \multirow{4}{*}{F1} & \ding{55} & \ding{51} & \bR$0.757_{0.048}$ \\
%                     & \ding{55} & \ding{55} &  $0.609_{0.119}$ \\\cmidrule(lr){2-3} \cmidrule(lr){4-4} \addlinespace[0.5ex]
%                     & \ding{51} & \ding{55} &  $0.695_{0.067}$ \\
%                     & \ding{51} & \ding{51} &  $0.753_{0.031}$ \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Using operation-wise hardware embedding to capture operation interactions as well as iniitalizing hardware embeddings with the closest correlated device improve performance.}
% \label{table:hw_mlp_hwinit}
% \end{table}

% \section{Introduction}

% Contributions
% \begin{itemize}
%     \item State of the art latency predictor with transfer learning support. Introduce concept of operation specific hardware embeddings. 
%     \item Demonstrating applicability of algorithm on micro and macro cell spaces (NB201 and FBNet).
%     \item Generate encodings (arch2vec, zcp etc) for FBNet and NASBench-201 and leverage them to create better network samplers.
%     \item Leveraging supplemental encodings to improve latency predictor performance. 
%     \item Designing difficult problems for effective evaluation of existing and our methodology. 
% \end{itemize}


% \section{Related Work}
% \subsection{Hardware Latency Predictors}
% From scratch research, then HELP, MultiPredict
% \subsection{Encodings for NN representation}
% MultiPredict, zcp, arch2vec, cate
% \subsection{Network Samplers}
% Literature review pending

% \section{Search Spaces}
% \subsection{Micro Cell Space (NASBench-201)}
% Describe what is micro.
% \subsection{Macro Cell Space (FBNet)}
% Describe what is macro and why we use it in this paper.


% \section{On Neural Network Samplers}
% \subsection{Neural Network Encodings}
% Describe Arch2Vec, CATE, ZCP
% \subsection{Leveraging Encodings For Selection}
% \begin{enumerate}
%     \item Demonstrate Eyeriss learning variance based on sampling (Find and reference the sampling paper, MAESTRO related?)
%     \item Show Uniform Sampling For Scalar Metrics
%     \item Show how to choose points from k-Means clustered vector encodings
% \end{enumerate}

% \subsection{Minimizing Pre-Training Samples}

% \begin{enumerate}
%     \item Why do we need to reduce pre-training sample count? : Prototyping search spaces for NAS
%     \item Discussion on task distance (MultiPredict)
% \end{enumerate}

% \subsection{Minimizing Pre-Training Devices}

% \begin{enumerate}
%     \item Importance of reducing number of devices -- lesser infrastructured
%     \item How do we choose devices -- we do not tackle this. But given NASBench-201 correlation, can we choose which devices to benchmark FBNet on? 
% \end{enumerate}


% \section{On Device Embeddings}
% \subsection{Global Hardware Embedding}
% Multi-Predict pipes HW Embeddings (Index, Sample, Learnable) to final MLP. Similar approach by HELP. 

% \subsection{Operation Specific Hardware Embedding}
% \begin{itemize}
%     \item Operation placement may have interactions, effecting the latency.
%     \item Concatenating a learnable hardware encoding with operation encoding may provide broader context for GNN.
% \end{itemize}

% \section{On Predictor Architectures}
% \subsection{MLP Predictors}
% HELP and MultiPredict use MLP for FBNet. NB201 can have flattened adj-op matrices.

% \subsection{Graph Neural Network Architecture}
% \textbf{Operations and Residual Connections}

% \begin{itemize}
%     \item Operation Embedding Update with MLP. Reference TAGATES and Appendix.
%     \item Residual Connections, Oversmoothing, Motivate GNN Module Design
% \end{itemize}

% \subsection{GNN Module Design}
% \begin{itemize}
%     \item GNN with residual support
%     \item Graph Attention Networks
% \end{itemize}

% \subsection{Supplementary Encodings}
% \begin{itemize}
%     \item Arch2Vec distinguished NN archs.
%     \item CATE param metric, ZCP gives properties
%     \item Combining them may provide more context for prediction
% \end{itemize}

% \section{Experiments}
% \subsection{Designing Evaluation Sets}
% \begin{itemize}
%     \item Min k-cut and Kernighan-Lin. (reference MultiPredict adversarial)
% \end{itemize}

% \subsection{Latency Predictor}
% First, evaluate predictors with Training from Scratch strategy on each test hardware for HELP, MultiPredict and Ours.

% \textbf{Does accuracy improve if we sample better networks when training from scratch?}

% \subsection{Encodings For Selection}
% Experiments on different methods of selecting NN architectures and their result/variance.

% \subsection{Encodings for Supplementing}
% Experiments on different methods of supplement NN information and their result/variance.

% \subsection{Pre-Training Samples and Devices}
% Experiments on accuracy as we reduce number of pre-training samples and devices, conducted for different supplemental encodings.

% \subsection{Transfer Of Latency Predictor}
% Experiments comparing our best selection + supplement + architecture strategy with HELP and MultiPredict on difficult device sets.






% \section{On Neural Network Samplers}
% \subsection{Neural Network Encodings}
% Describe Arch2Vec, CATE, ZCP.
% \subsection{Leveraging Encodings for Selection}
% Describe uniform sorted sampling for scalar metrics, K-Means centroid selection strategy for vector metrics. 

% \textbf{Table 1: NB201 and FBNet Sampling Methods vs. Variance (or correlation itself)}

% \subsection{Minimizing Pre-Training Samples}

% Describe the need for reducing the samples required for pre-training. (Task distance matters (Multi-Predict)), if a new reference hardware is required for pre-training, it is efficient to reduce samples required. (Issue: If you have 10 samples, is it really that hard to get 100? \textit{Maybe if you are prototyping macro spaces?}) 

% \textbf{Table 2: NB201 and FBNet test how accuracy falls as num samples fall for a difficult task.}

% \subsection{Minimizing Pre-Training Devices}
% Figuring out which devices you need, or what is the minimal device set translates to lesser overhead in infrastructure. However, if a few samples are gathered, is it really that difficult to gather more? How do we decide how many are required? (Unclear, we do not solve this). We can still look at what happens as we reduce num devices slowly.

% \textbf{Table 3: NB201 and FBNet take a device set, make it increasingly harder and see scaling as devices decrease.}
% \textit{Table 4: NB201 and FBNet instead of taking a device set and removing high corr devices, remove random.}

% \section{On Device Embeddings}
% \subsection{Global Hardware Embedding}
% MultiPredict pipes HW Embedding to final MLP
% \subsection{Operation Specific Hardware Embedding}
% Operations placed after one another may have pipelining characteristics etc which require neighbourhood communication. Maybe we can benefit from concatenating operation and hardware information and using that in GNN.

% \textbf{Table 5: NB201 and FBNet on device sets, with and without op-specific hw embedding.}

% \section{On Predictor Architectures}
% \subsection{MLP Predictors}
% HELP and MultiPredict use MLP for FBNet. NB201 can have flattened adj-op mat
% \textbf{Table 6: NB201 and FBNet MLP vs GCN}
% \subsection{Graph Neural Network Architecture}
% Residual, Graph Attention
% \subsection{Operation Embeddings}
% Operation - Hardware Embedding Update
% \textbf{Table 7 (Appx?): Design Choices and KDT}
% \subsection{Supplementary Encodings}
% \textbf{Table 8: FBNet and NB201 Supplementing arch2vec, CATE, ZCP}
% \section{On Transfer Learning}
% \subsection{Minimum k-cut and Hardware Distance}
% Describe Min k-cut and Kernighan-Lin for finding difficult tasks (follow up on MultiPredict).
% \subsection{Generalized Performance}
% Discuss whether generalizable performance is required, or is it better to just adapt a network? (Maybe exclude)
% \subsection{Hardware Specific Performance}
% Training from scratch vs transfer learning. 
% \subsection{}

% \subsection{}

% \begin{algorithm}[tb]
%    \caption{Bubble Sort}
%    \label{alg:example}
% \begin{algorithmic}
%    \STATE {\bfseries Input:} data $x_i$, size $m$
%    \REPEAT
%    \STATE Initialize $noChange = true$.
%    \FOR{$i=1$ {\bfseries to} $m-1$}
%    \IF{$x_i > x_{i+1}$}
%    \STATE Swap $x_i$ and $x_{i+1}$
%    \STATE $noChange = false$
%    \ENDIF
%    \ENDFOR
%    \UNTIL{$noChange$ is $true$}
% \end{algorithmic}
% \end{algorithm}

% \begin{table}[t]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Data set & Naive & Flexible & Better? \\
% \midrule
% Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
% Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
% Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
% Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
% Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
% Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
% Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}
% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite
